Search for charged Higgs bosons decaying via $H^{\pm} \rightarrow \tau^{\pm}\nu$ in fully hadronic final states using $pp$ collision data at $\sqrt{s} = 8$ TeV with the ATLAS detector

The results of a search for charged Higgs bosons decaying to a $\tau$ lepton and a neutrino, $H^{\pm} \rightarrow \tau^{\pm} \nu$, are presented. The analysis is based on 19.5 fb$^{-1}$ of proton-proton collision data at $\sqrt{s}=8$ TeV collected by the ATLAS experiment at the Large Hadron Collider. Charged Higgs bosons are searched for in events consistent with top-quark pair production or in associated production with a top quark. The final state is characterised by the presence of a hadronic $\tau$ decay, missing transverse momentum, $b$-tagged jets, a hadronically decaying $W$ boson, and the absence of any isolated electrons or muons with high transverse momenta. The data are consistent with the expected background from Standard Model processes. A statistical analysis leads to 95\% confidence-level upper limits on the product of branching ratios $ {\cal B}(t\rightarrow bH^\pm) \times {\cal B} (H^\pm\rightarrow \tau^{\pm}\nu) $, between 0.23% and 1.3% for charged Higgs boson masses in the range 80-160 GeV. It also leads to 95% confidence-level upper limits on the production cross section times branching ratio, $\sigma(pp \rightarrow tH^{\pm} + X) \times {\cal B}(H^{\pm} \rightarrow \tau^{\pm} \nu)$, between 0.76 pb and 4.5 fb, for charged Higgs boson masses ranging from 180 GeV to 1000 GeV. In the context of different scenarios of the Minimal Supersymmetric Standard Model, these results exclude nearly all values of $\tan\beta$ above one for charged Higgs boson masses between 80 GeV and 160 GeV, and exclude a region of parameter space with high $\tan\beta$ for $H^{\pm}$ masses between 200 GeV and 250 GeV.

==> Additions.tex <==
Since first circulation we added scenario-specific MSSM interpretation plots of our
results. The analysis itself has not changed and everything up to the branching ratio/
cross section limits is the same as documented in ATLAS-CONF-2014-050. Figure 8 has
been added, including explanations in the results section. The abstract and conclusions
have been updated accordingly to incorporate the new results.


==> old_atlas_authlist.tex <==
% ATLAS Collaboration author list
% Data extracted on 19-Dec-2014 for paper reference HIGG-2013-30
%% \documentclass[11pt]{article}
%% \usepackage{a4wide}\begin{document}
\begin{flushleft}
{\Large The ATLAS Collaboration}

\bigskip

G.~Aad$^{\rm 85}$,
B.~Abbott$^{\rm 113}$,
J.~Abdallah$^{\rm 152}$,
O.~Abdinov$^{\rm 11}$,
R.~Aben$^{\rm 107}$,
M.~Abolins$^{\rm 90}$,
O.S.~AbouZeid$^{\rm 159}$,
H.~Abramowicz$^{\rm 154}$,
H.~Abreu$^{\rm 153}$,
R.~Abreu$^{\rm 30}$,
Y.~Abulaiti$^{\rm 147a,147b}$,
B.S.~Acharya$^{\rm 165a,165b}$$^{,a}$,
L.~Adamczyk$^{\rm 38a}$,
D.L.~Adams$^{\rm 25}$,
J.~Adelman$^{\rm 108}$,
S.~Adomeit$^{\rm 100}$,
T.~Adye$^{\rm 131}$,
T.~Agatonovic-Jovin$^{\rm 13}$,
J.A.~Aguilar-Saavedra$^{\rm 126a,126f}$,
M.~Agustoni$^{\rm 17}$,
S.P.~Ahlen$^{\rm 22}$,
F.~Ahmadov$^{\rm 65}$$^{,b}$,
G.~Aielli$^{\rm 134a,134b}$,
H.~Akerstedt$^{\rm 147a,147b}$,
T.P.A.~{\AA}kesson$^{\rm 81}$,
G.~Akimoto$^{\rm 156}$,
A.V.~Akimov$^{\rm 96}$,
G.L.~Alberghi$^{\rm 20a,20b}$,
J.~Albert$^{\rm 170}$,
S.~Albrand$^{\rm 55}$,
M.J.~Alconada~Verzini$^{\rm 71}$,
M.~Aleksa$^{\rm 30}$,
I.N.~Aleksandrov$^{\rm 65}$,
C.~Alexa$^{\rm 26a}$,
G.~Alexander$^{\rm 154}$,
T.~Alexopoulos$^{\rm 10}$,
M.~Alhroob$^{\rm 113}$,
G.~Alimonti$^{\rm 91a}$,
L.~Alio$^{\rm 85}$,
J.~Alison$^{\rm 31}$,
B.M.M.~Allbrooke$^{\rm 18}$,
P.P.~Allport$^{\rm 74}$,
A.~Aloisio$^{\rm 104a,104b}$,
A.~Alonso$^{\rm 36}$,
F.~Alonso$^{\rm 71}$,
C.~Alpigiani$^{\rm 76}$,
A.~Altheimer$^{\rm 35}$,
B.~Alvarez~Gonzalez$^{\rm 90}$,
M.G.~Alviggi$^{\rm 104a,104b}$,
K.~Amako$^{\rm 66}$,
Y.~Amaral~Coutinho$^{\rm 24a}$,
C.~Amelung$^{\rm 23}$,
D.~Amidei$^{\rm 89}$,
S.P.~Amor~Dos~Santos$^{\rm 126a,126c}$,
A.~Amorim$^{\rm 126a,126b}$,
S.~Amoroso$^{\rm 48}$,
N.~Amram$^{\rm 154}$,
G.~Amundsen$^{\rm 23}$,
C.~Anastopoulos$^{\rm 140}$,
L.S.~Ancu$^{\rm 49}$,
N.~Andari$^{\rm 30}$,
T.~Andeen$^{\rm 35}$,
C.F.~Anders$^{\rm 58b}$,
G.~Anders$^{\rm 30}$,
K.J.~Anderson$^{\rm 31}$,
A.~Andreazza$^{\rm 91a,91b}$,
V.~Andrei$^{\rm 58a}$,
X.S.~Anduaga$^{\rm 71}$,
S.~Angelidakis$^{\rm 9}$,
I.~Angelozzi$^{\rm 107}$,
P.~Anger$^{\rm 44}$,
A.~Angerami$^{\rm 35}$,
F.~Anghinolfi$^{\rm 30}$,
A.V.~Anisenkov$^{\rm 109}$$^{,c}$,
N.~Anjos$^{\rm 12}$,
A.~Annovi$^{\rm 124a,124b}$,
M.~Antonelli$^{\rm 47}$,
A.~Antonov$^{\rm 98}$,
J.~Antos$^{\rm 145b}$,
F.~Anulli$^{\rm 133a}$,
M.~Aoki$^{\rm 66}$,
L.~Aperio~Bella$^{\rm 18}$,
G.~Arabidze$^{\rm 90}$,
Y.~Arai$^{\rm 66}$,
J.P.~Araque$^{\rm 126a}$,
A.T.H.~Arce$^{\rm 45}$,
F.A.~Arduh$^{\rm 71}$,
J-F.~Arguin$^{\rm 95}$,
S.~Argyropoulos$^{\rm 42}$,
M.~Arik$^{\rm 19a}$,
A.J.~Armbruster$^{\rm 30}$,
O.~Arnaez$^{\rm 30}$,
V.~Arnal$^{\rm 82}$,
H.~Arnold$^{\rm 48}$,
M.~Arratia$^{\rm 28}$,
O.~Arslan$^{\rm 21}$,
A.~Artamonov$^{\rm 97}$,
G.~Artoni$^{\rm 23}$,
S.~Asai$^{\rm 156}$,
N.~Asbah$^{\rm 42}$,
A.~Ashkenazi$^{\rm 154}$,
B.~{\AA}sman$^{\rm 147a,147b}$,
L.~Asquith$^{\rm 150}$,
K.~Assamagan$^{\rm 25}$,
R.~Astalos$^{\rm 145a}$,
M.~Atkinson$^{\rm 166}$,
N.B.~Atlay$^{\rm 142}$,
B.~Auerbach$^{\rm 6}$,
K.~Augsten$^{\rm 128}$,
M.~Aurousseau$^{\rm 146b}$,
G.~Avolio$^{\rm 30}$,
B.~Axen$^{\rm 15}$,
M.K.~Ayoub$^{\rm 117}$,
G.~Azuelos$^{\rm 95}$$^{,d}$,
M.A.~Baak$^{\rm 30}$,
A.E.~Baas$^{\rm 58a}$,
C.~Bacci$^{\rm 135a,135b}$,
H.~Bachacou$^{\rm 137}$,
K.~Bachas$^{\rm 155}$,
M.~Backes$^{\rm 30}$,
M.~Backhaus$^{\rm 30}$,
E.~Badescu$^{\rm 26a}$,
P.~Bagiacchi$^{\rm 133a,133b}$,
P.~Bagnaia$^{\rm 133a,133b}$,
Y.~Bai$^{\rm 33a}$,
T.~Bain$^{\rm 35}$,
J.T.~Baines$^{\rm 131}$,
O.K.~Baker$^{\rm 177}$,
P.~Balek$^{\rm 129}$,
T.~Balestri$^{\rm 149}$,
F.~Balli$^{\rm 84}$,
E.~Banas$^{\rm 39}$,
Sw.~Banerjee$^{\rm 174}$,
A.A.E.~Bannoura$^{\rm 176}$,
H.S.~Bansil$^{\rm 18}$,
L.~Barak$^{\rm 30}$,
S.P.~Baranov$^{\rm 96}$,
E.L.~Barberio$^{\rm 88}$,
D.~Barberis$^{\rm 50a,50b}$,
M.~Barbero$^{\rm 85}$,
T.~Barillari$^{\rm 101}$,
M.~Barisonzi$^{\rm 165a,165b}$,
T.~Barklow$^{\rm 144}$,
N.~Barlow$^{\rm 28}$,
S.L.~Barnes$^{\rm 84}$,
B.M.~Barnett$^{\rm 131}$,
R.M.~Barnett$^{\rm 15}$,
Z.~Barnovska$^{\rm 5}$,
A.~Baroncelli$^{\rm 135a}$,
G.~Barone$^{\rm 49}$,
A.J.~Barr$^{\rm 120}$,
F.~Barreiro$^{\rm 82}$,
J.~Barreiro~Guimar\~{a}es~da~Costa$^{\rm 57}$,
R.~Bartoldus$^{\rm 144}$,
A.E.~Barton$^{\rm 72}$,
P.~Bartos$^{\rm 145a}$,
A.~Bassalat$^{\rm 117}$,
A.~Basye$^{\rm 166}$,
R.L.~Bates$^{\rm 53}$,
S.J.~Batista$^{\rm 159}$,
J.R.~Batley$^{\rm 28}$,
M.~Battaglia$^{\rm 138}$,
M.~Bauce$^{\rm 133a,133b}$,
F.~Bauer$^{\rm 137}$,
H.S.~Bawa$^{\rm 144}$$^{,e}$,
J.B.~Beacham$^{\rm 111}$,
M.D.~Beattie$^{\rm 72}$,
T.~Beau$^{\rm 80}$,
P.H.~Beauchemin$^{\rm 162}$,
R.~Beccherle$^{\rm 124a,124b}$,
P.~Bechtle$^{\rm 21}$,
H.P.~Beck$^{\rm 17}$$^{,f}$,
K.~Becker$^{\rm 120}$,
S.~Becker$^{\rm 100}$,
M.~Beckingham$^{\rm 171}$,
C.~Becot$^{\rm 117}$,
A.J.~Beddall$^{\rm 19c}$,
A.~Beddall$^{\rm 19c}$,
V.A.~Bednyakov$^{\rm 65}$,
C.P.~Bee$^{\rm 149}$,
L.J.~Beemster$^{\rm 107}$,
T.A.~Beermann$^{\rm 176}$,
M.~Begel$^{\rm 25}$,
K.~Behr$^{\rm 120}$,
C.~Belanger-Champagne$^{\rm 87}$,
P.J.~Bell$^{\rm 49}$,
W.H.~Bell$^{\rm 49}$,
G.~Bella$^{\rm 154}$,
L.~Bellagamba$^{\rm 20a}$,
A.~Bellerive$^{\rm 29}$,
M.~Bellomo$^{\rm 86}$,
K.~Belotskiy$^{\rm 98}$,
O.~Beltramello$^{\rm 30}$,
O.~Benary$^{\rm 154}$,
D.~Benchekroun$^{\rm 136a}$,
M.~Bender$^{\rm 100}$,
K.~Bendtz$^{\rm 147a,147b}$,
N.~Benekos$^{\rm 10}$,
Y.~Benhammou$^{\rm 154}$,
E.~Benhar~Noccioli$^{\rm 49}$,
J.A.~Benitez~Garcia$^{\rm 160b}$,
D.P.~Benjamin$^{\rm 45}$,
J.R.~Bensinger$^{\rm 23}$,
S.~Bentvelsen$^{\rm 107}$,
L.~Beresford$^{\rm 120}$,
M.~Beretta$^{\rm 47}$,
D.~Berge$^{\rm 107}$,
E.~Bergeaas~Kuutmann$^{\rm 167}$,
N.~Berger$^{\rm 5}$,
F.~Berghaus$^{\rm 170}$,
J.~Beringer$^{\rm 15}$,
C.~Bernard$^{\rm 22}$,
N.R.~Bernard$^{\rm 86}$,
C.~Bernius$^{\rm 110}$,
F.U.~Bernlochner$^{\rm 21}$,
T.~Berry$^{\rm 77}$,
P.~Berta$^{\rm 129}$,
C.~Bertella$^{\rm 83}$,
G.~Bertoli$^{\rm 147a,147b}$,
F.~Bertolucci$^{\rm 124a,124b}$,
C.~Bertsche$^{\rm 113}$,
D.~Bertsche$^{\rm 113}$,
M.I.~Besana$^{\rm 91a}$,
G.J.~Besjes$^{\rm 106}$,
O.~Bessidskaia$^{\rm 147a,147b}$,
M.~Bessner$^{\rm 42}$,
N.~Besson$^{\rm 137}$,
C.~Betancourt$^{\rm 48}$,
S.~Bethke$^{\rm 101}$,
A.J.~Bevan$^{\rm 76}$,
W.~Bhimji$^{\rm 46}$,
R.M.~Bianchi$^{\rm 125}$,
L.~Bianchini$^{\rm 23}$,
M.~Bianco$^{\rm 30}$,
O.~Biebel$^{\rm 100}$,
S.P.~Bieniek$^{\rm 78}$,
M.~Biglietti$^{\rm 135a}$,
J.~Bilbao~De~Mendizabal$^{\rm 49}$,
H.~Bilokon$^{\rm 47}$,
M.~Bindi$^{\rm 54}$,
S.~Binet$^{\rm 117}$,
A.~Bingul$^{\rm 19c}$,
C.~Bini$^{\rm 133a,133b}$,
C.W.~Black$^{\rm 151}$,
J.E.~Black$^{\rm 144}$,
K.M.~Black$^{\rm 22}$,
D.~Blackburn$^{\rm 139}$,
R.E.~Blair$^{\rm 6}$,
J.-B.~Blanchard$^{\rm 137}$,
J.E.~Blanco$^{\rm 77}$,
T.~Blazek$^{\rm 145a}$,
I.~Bloch$^{\rm 42}$,
C.~Blocker$^{\rm 23}$,
W.~Blum$^{\rm 83}$$^{,*}$,
U.~Blumenschein$^{\rm 54}$,
G.J.~Bobbink$^{\rm 107}$,
V.S.~Bobrovnikov$^{\rm 109}$$^{,c}$,
S.S.~Bocchetta$^{\rm 81}$,
A.~Bocci$^{\rm 45}$,
C.~Bock$^{\rm 100}$,
M.~Boehler$^{\rm 48}$,
J.A.~Bogaerts$^{\rm 30}$,
A.G.~Bogdanchikov$^{\rm 109}$,
C.~Bohm$^{\rm 147a}$,
V.~Boisvert$^{\rm 77}$,
T.~Bold$^{\rm 38a}$,
V.~Boldea$^{\rm 26a}$,
A.S.~Boldyrev$^{\rm 99}$,
M.~Bomben$^{\rm 80}$,
M.~Bona$^{\rm 76}$,
M.~Boonekamp$^{\rm 137}$,
A.~Borisov$^{\rm 130}$,
G.~Borissov$^{\rm 72}$,
S.~Borroni$^{\rm 42}$,
J.~Bortfeldt$^{\rm 100}$,
V.~Bortolotto$^{\rm 60a,60b,60c}$,
K.~Bos$^{\rm 107}$,
D.~Boscherini$^{\rm 20a}$,
M.~Bosman$^{\rm 12}$,
J.~Boudreau$^{\rm 125}$,
J.~Bouffard$^{\rm 2}$,
E.V.~Bouhova-Thacker$^{\rm 72}$,
D.~Boumediene$^{\rm 34}$,
C.~Bourdarios$^{\rm 117}$,
N.~Bousson$^{\rm 114}$,
S.~Boutouil$^{\rm 136d}$,
A.~Boveia$^{\rm 30}$,
J.~Boyd$^{\rm 30}$,
I.R.~Boyko$^{\rm 65}$,
I.~Bozic$^{\rm 13}$,
J.~Bracinik$^{\rm 18}$,
A.~Brandt$^{\rm 8}$,
G.~Brandt$^{\rm 15}$,
O.~Brandt$^{\rm 58a}$,
U.~Bratzler$^{\rm 157}$,
B.~Brau$^{\rm 86}$,
J.E.~Brau$^{\rm 116}$,
H.M.~Braun$^{\rm 176}$$^{,*}$,
S.F.~Brazzale$^{\rm 165a,165c}$,
K.~Brendlinger$^{\rm 122}$,
A.J.~Brennan$^{\rm 88}$,
L.~Brenner$^{\rm 107}$,
R.~Brenner$^{\rm 167}$,
S.~Bressler$^{\rm 173}$,
K.~Bristow$^{\rm 146c}$,
T.M.~Bristow$^{\rm 46}$,
D.~Britton$^{\rm 53}$,
D.~Britzger$^{\rm 42}$,
F.M.~Brochu$^{\rm 28}$,
I.~Brock$^{\rm 21}$,
R.~Brock$^{\rm 90}$,
J.~Bronner$^{\rm 101}$,
G.~Brooijmans$^{\rm 35}$,
T.~Brooks$^{\rm 77}$,
W.K.~Brooks$^{\rm 32b}$,
J.~Brosamer$^{\rm 15}$,
E.~Brost$^{\rm 116}$,
J.~Brown$^{\rm 55}$,
P.A.~Bruckman~de~Renstrom$^{\rm 39}$,
D.~Bruncko$^{\rm 145b}$,
R.~Bruneliere$^{\rm 48}$,
A.~Bruni$^{\rm 20a}$,
G.~Bruni$^{\rm 20a}$,
M.~Bruschi$^{\rm 20a}$,
L.~Bryngemark$^{\rm 81}$,
T.~Buanes$^{\rm 14}$,
Q.~Buat$^{\rm 143}$,
P.~Buchholz$^{\rm 142}$,
A.G.~Buckley$^{\rm 53}$,
S.I.~Buda$^{\rm 26a}$,
I.A.~Budagov$^{\rm 65}$,
F.~Buehrer$^{\rm 48}$,
L.~Bugge$^{\rm 119}$,
M.K.~Bugge$^{\rm 119}$,
O.~Bulekov$^{\rm 98}$,
H.~Burckhart$^{\rm 30}$,
S.~Burdin$^{\rm 74}$,
B.~Burghgrave$^{\rm 108}$,
S.~Burke$^{\rm 131}$,
I.~Burmeister$^{\rm 43}$,
E.~Busato$^{\rm 34}$,
D.~B\"uscher$^{\rm 48}$,
V.~B\"uscher$^{\rm 83}$,
P.~Bussey$^{\rm 53}$,
C.P.~Buszello$^{\rm 167}$,
J.M.~Butler$^{\rm 22}$,
A.I.~Butt$^{\rm 3}$,
C.M.~Buttar$^{\rm 53}$,
J.M.~Butterworth$^{\rm 78}$,
P.~Butti$^{\rm 107}$,
W.~Buttinger$^{\rm 25}$,
A.~Buzatu$^{\rm 53}$,
S.~Cabrera~Urb\'an$^{\rm 168}$,
D.~Caforio$^{\rm 128}$,
O.~Cakir$^{\rm 4a}$,
P.~Calafiura$^{\rm 15}$,
A.~Calandri$^{\rm 137}$,
G.~Calderini$^{\rm 80}$,
P.~Calfayan$^{\rm 100}$,
L.P.~Caloba$^{\rm 24a}$,
D.~Calvet$^{\rm 34}$,
S.~Calvet$^{\rm 34}$,
R.~Camacho~Toro$^{\rm 49}$,
S.~Camarda$^{\rm 42}$,
D.~Cameron$^{\rm 119}$,
L.M.~Caminada$^{\rm 15}$,
R.~Caminal~Armadans$^{\rm 12}$,
S.~Campana$^{\rm 30}$,
M.~Campanelli$^{\rm 78}$,
A.~Campoverde$^{\rm 149}$,
V.~Canale$^{\rm 104a,104b}$,
A.~Canepa$^{\rm 160a}$,
M.~Cano~Bret$^{\rm 76}$,
J.~Cantero$^{\rm 82}$,
R.~Cantrill$^{\rm 126a}$,
T.~Cao$^{\rm 40}$,
M.D.M.~Capeans~Garrido$^{\rm 30}$,
I.~Caprini$^{\rm 26a}$,
M.~Caprini$^{\rm 26a}$,
M.~Capua$^{\rm 37a,37b}$,
R.~Caputo$^{\rm 83}$,
R.~Cardarelli$^{\rm 134a}$,
T.~Carli$^{\rm 30}$,
G.~Carlino$^{\rm 104a}$,
L.~Carminati$^{\rm 91a,91b}$,
S.~Caron$^{\rm 106}$,
E.~Carquin$^{\rm 32a}$,
G.D.~Carrillo-Montoya$^{\rm 8}$,
J.R.~Carter$^{\rm 28}$,
J.~Carvalho$^{\rm 126a,126c}$,
D.~Casadei$^{\rm 78}$,
M.P.~Casado$^{\rm 12}$,
M.~Casolino$^{\rm 12}$,
E.~Castaneda-Miranda$^{\rm 146b}$,
A.~Castelli$^{\rm 107}$,
V.~Castillo~Gimenez$^{\rm 168}$,
N.F.~Castro$^{\rm 126a}$,
P.~Catastini$^{\rm 57}$,
A.~Catinaccio$^{\rm 30}$,
J.R.~Catmore$^{\rm 119}$,
A.~Cattai$^{\rm 30}$,
J.~Caudron$^{\rm 83}$,
V.~Cavaliere$^{\rm 166}$,
D.~Cavalli$^{\rm 91a}$,
M.~Cavalli-Sforza$^{\rm 12}$,
V.~Cavasinni$^{\rm 124a,124b}$,
F.~Ceradini$^{\rm 135a,135b}$,
B.C.~Cerio$^{\rm 45}$,
K.~Cerny$^{\rm 129}$,
A.S.~Cerqueira$^{\rm 24b}$,
A.~Cerri$^{\rm 150}$,
L.~Cerrito$^{\rm 76}$,
F.~Cerutti$^{\rm 15}$,
M.~Cerv$^{\rm 30}$,
A.~Cervelli$^{\rm 17}$,
S.A.~Cetin$^{\rm 19b}$,
A.~Chafaq$^{\rm 136a}$,
D.~Chakraborty$^{\rm 108}$,
I.~Chalupkova$^{\rm 129}$,
P.~Chang$^{\rm 166}$,
B.~Chapleau$^{\rm 87}$,
J.D.~Chapman$^{\rm 28}$,
D.G.~Charlton$^{\rm 18}$,
C.C.~Chau$^{\rm 159}$,
C.A.~Chavez~Barajas$^{\rm 150}$,
S.~Cheatham$^{\rm 153}$,
A.~Chegwidden$^{\rm 90}$,
S.~Chekanov$^{\rm 6}$,
S.V.~Chekulaev$^{\rm 160a}$,
G.A.~Chelkov$^{\rm 65}$$^{,g}$,
M.A.~Chelstowska$^{\rm 89}$,
C.~Chen$^{\rm 64}$,
H.~Chen$^{\rm 25}$,
K.~Chen$^{\rm 149}$,
L.~Chen$^{\rm 33d}$$^{,h}$,
S.~Chen$^{\rm 33c}$,
X.~Chen$^{\rm 33f}$,
Y.~Chen$^{\rm 67}$,
H.C.~Cheng$^{\rm 89}$,
Y.~Cheng$^{\rm 31}$,
A.~Cheplakov$^{\rm 65}$,
E.~Cheremushkina$^{\rm 130}$,
R.~Cherkaoui~El~Moursli$^{\rm 136e}$,
V.~Chernyatin$^{\rm 25}$$^{,*}$,
E.~Cheu$^{\rm 7}$,
L.~Chevalier$^{\rm 137}$,
V.~Chiarella$^{\rm 47}$,
J.T.~Childers$^{\rm 6}$,
A.~Chilingarov$^{\rm 72}$,
G.~Chiodini$^{\rm 73a}$,
A.S.~Chisholm$^{\rm 18}$,
R.T.~Chislett$^{\rm 78}$,
A.~Chitan$^{\rm 26a}$,
M.V.~Chizhov$^{\rm 65}$,
K.~Choi$^{\rm 61}$,
S.~Chouridou$^{\rm 9}$,
B.K.B.~Chow$^{\rm 100}$,
V.~Christodoulou$^{\rm 78}$,
D.~Chromek-Burckhart$^{\rm 30}$,
M.L.~Chu$^{\rm 152}$,
J.~Chudoba$^{\rm 127}$,
J.J.~Chwastowski$^{\rm 39}$,
L.~Chytka$^{\rm 115}$,
G.~Ciapetti$^{\rm 133a,133b}$,
A.K.~Ciftci$^{\rm 4a}$,
D.~Cinca$^{\rm 53}$,
V.~Cindro$^{\rm 75}$,
A.~Ciocio$^{\rm 15}$,
Z.H.~Citron$^{\rm 173}$,
M.~Citterio$^{\rm 91a}$,
M.~Ciubancan$^{\rm 26a}$,
A.~Clark$^{\rm 49}$,
B.L.~Clark$^{\rm 57}$,
P.J.~Clark$^{\rm 46}$,
R.N.~Clarke$^{\rm 15}$,
W.~Cleland$^{\rm 125}$,
C.~Clement$^{\rm 147a,147b}$,
Y.~Coadou$^{\rm 85}$,
M.~Cobal$^{\rm 165a,165c}$,
A.~Coccaro$^{\rm 139}$,
J.~Cochran$^{\rm 64}$,
L.~Coffey$^{\rm 23}$,
J.G.~Cogan$^{\rm 144}$,
B.~Cole$^{\rm 35}$,
S.~Cole$^{\rm 108}$,
A.P.~Colijn$^{\rm 107}$,
J.~Collot$^{\rm 55}$,
T.~Colombo$^{\rm 58c}$,
G.~Compostella$^{\rm 101}$,
P.~Conde~Mui\~no$^{\rm 126a,126b}$,
E.~Coniavitis$^{\rm 48}$,
S.H.~Connell$^{\rm 146b}$,
I.A.~Connelly$^{\rm 77}$,
S.M.~Consonni$^{\rm 91a,91b}$,
V.~Consorti$^{\rm 48}$,
S.~Constantinescu$^{\rm 26a}$,
C.~Conta$^{\rm 121a,121b}$,
G.~Conti$^{\rm 30}$,
F.~Conventi$^{\rm 104a}$$^{,i}$,
M.~Cooke$^{\rm 15}$,
B.D.~Cooper$^{\rm 78}$,
A.M.~Cooper-Sarkar$^{\rm 120}$,
K.~Copic$^{\rm 15}$,
T.~Cornelissen$^{\rm 176}$,
M.~Corradi$^{\rm 20a}$,
F.~Corriveau$^{\rm 87}$$^{,j}$,
A.~Corso-Radu$^{\rm 164}$,
A.~Cortes-Gonzalez$^{\rm 12}$,
G.~Cortiana$^{\rm 101}$,
M.J.~Costa$^{\rm 168}$,
D.~Costanzo$^{\rm 140}$,
D.~C\^ot\'e$^{\rm 8}$,
G.~Cottin$^{\rm 28}$,
G.~Cowan$^{\rm 77}$,
B.E.~Cox$^{\rm 84}$,
K.~Cranmer$^{\rm 110}$,
G.~Cree$^{\rm 29}$,
S.~Cr\'ep\'e-Renaudin$^{\rm 55}$,
F.~Crescioli$^{\rm 80}$,
W.A.~Cribbs$^{\rm 147a,147b}$,
M.~Crispin~Ortuzar$^{\rm 120}$,
M.~Cristinziani$^{\rm 21}$,
V.~Croft$^{\rm 106}$,
G.~Crosetti$^{\rm 37a,37b}$,
T.~Cuhadar~Donszelmann$^{\rm 140}$,
J.~Cummings$^{\rm 177}$,
M.~Curatolo$^{\rm 47}$,
C.~Cuthbert$^{\rm 151}$,
H.~Czirr$^{\rm 142}$,
P.~Czodrowski$^{\rm 3}$,
S.~D'Auria$^{\rm 53}$,
M.~D'Onofrio$^{\rm 74}$,
M.J.~Da~Cunha~Sargedas~De~Sousa$^{\rm 126a,126b}$,
C.~Da~Via$^{\rm 84}$,
W.~Dabrowski$^{\rm 38a}$,
A.~Dafinca$^{\rm 120}$,
T.~Dai$^{\rm 89}$,
O.~Dale$^{\rm 14}$,
F.~Dallaire$^{\rm 95}$,
C.~Dallapiccola$^{\rm 86}$,
M.~Dam$^{\rm 36}$,
J.R.~Dandoy$^{\rm 31}$,
A.C.~Daniells$^{\rm 18}$,
M.~Danninger$^{\rm 169}$,
M.~Dano~Hoffmann$^{\rm 137}$,
V.~Dao$^{\rm 48}$,
G.~Darbo$^{\rm 50a}$,
S.~Darmora$^{\rm 8}$,
J.~Dassoulas$^{\rm 3}$,
A.~Dattagupta$^{\rm 61}$,
W.~Davey$^{\rm 21}$,
C.~David$^{\rm 170}$,
T.~Davidek$^{\rm 129}$,
E.~Davies$^{\rm 120}$$^{,k}$,
M.~Davies$^{\rm 154}$,
P.~Davison$^{\rm 78}$,
Y.~Davygora$^{\rm 58a}$,
E.~Dawe$^{\rm 143}$,
I.~Dawson$^{\rm 140}$,
R.K.~Daya-Ishmukhametova$^{\rm 86}$,
K.~De$^{\rm 8}$,
R.~de~Asmundis$^{\rm 104a}$,
S.~De~Castro$^{\rm 20a,20b}$,
S.~De~Cecco$^{\rm 80}$,
N.~De~Groot$^{\rm 106}$,
P.~de~Jong$^{\rm 107}$,
H.~De~la~Torre$^{\rm 82}$,
F.~De~Lorenzi$^{\rm 64}$,
L.~De~Nooij$^{\rm 107}$,
D.~De~Pedis$^{\rm 133a}$,
A.~De~Salvo$^{\rm 133a}$,
U.~De~Sanctis$^{\rm 150}$,
A.~De~Santo$^{\rm 150}$,
J.B.~De~Vivie~De~Regie$^{\rm 117}$,
W.J.~Dearnaley$^{\rm 72}$,
R.~Debbe$^{\rm 25}$,
C.~Debenedetti$^{\rm 138}$,
D.V.~Dedovich$^{\rm 65}$,
I.~Deigaard$^{\rm 107}$,
J.~Del~Peso$^{\rm 82}$,
T.~Del~Prete$^{\rm 124a,124b}$,
D.~Delgove$^{\rm 117}$,
F.~Deliot$^{\rm 137}$,
C.M.~Delitzsch$^{\rm 49}$,
M.~Deliyergiyev$^{\rm 75}$,
A.~Dell'Acqua$^{\rm 30}$,
L.~Dell'Asta$^{\rm 22}$,
M.~Dell'Orso$^{\rm 124a,124b}$,
M.~Della~Pietra$^{\rm 104a}$$^{,i}$,
D.~della~Volpe$^{\rm 49}$,
M.~Delmastro$^{\rm 5}$,
P.A.~Delsart$^{\rm 55}$,
C.~Deluca$^{\rm 107}$,
D.A.~DeMarco$^{\rm 159}$,
S.~Demers$^{\rm 177}$,
M.~Demichev$^{\rm 65}$,
A.~Demilly$^{\rm 80}$,
S.P.~Denisov$^{\rm 130}$,
D.~Derendarz$^{\rm 39}$,
J.E.~Derkaoui$^{\rm 136d}$,
F.~Derue$^{\rm 80}$,
P.~Dervan$^{\rm 74}$,
K.~Desch$^{\rm 21}$,
C.~Deterre$^{\rm 42}$,
P.O.~Deviveiros$^{\rm 30}$,
A.~Dewhurst$^{\rm 131}$,
S.~Dhaliwal$^{\rm 107}$,
A.~Di~Ciaccio$^{\rm 134a,134b}$,
L.~Di~Ciaccio$^{\rm 5}$,
A.~Di~Domenico$^{\rm 133a,133b}$,
C.~Di~Donato$^{\rm 104a,104b}$,
A.~Di~Girolamo$^{\rm 30}$,
B.~Di~Girolamo$^{\rm 30}$,
A.~Di~Mattia$^{\rm 153}$,
B.~Di~Micco$^{\rm 135a,135b}$,
R.~Di~Nardo$^{\rm 47}$,
A.~Di~Simone$^{\rm 48}$,
R.~Di~Sipio$^{\rm 159}$,
D.~Di~Valentino$^{\rm 29}$,
C.~Diaconu$^{\rm 85}$,
M.~Diamond$^{\rm 159}$,
F.A.~Dias$^{\rm 46}$,
M.A.~Diaz$^{\rm 32a}$,
E.B.~Diehl$^{\rm 89}$,
J.~Dietrich$^{\rm 16}$,
S.~Diglio$^{\rm 85}$,
A.~Dimitrievska$^{\rm 13}$,
J.~Dingfelder$^{\rm 21}$,
F.~Dittus$^{\rm 30}$,
F.~Djama$^{\rm 85}$,
T.~Djobava$^{\rm 51b}$,
J.I.~Djuvsland$^{\rm 58a}$,
M.A.B.~do~Vale$^{\rm 24c}$,
D.~Dobos$^{\rm 30}$,
M.~Dobre$^{\rm 26a}$,
C.~Doglioni$^{\rm 49}$,
T.~Dohmae$^{\rm 156}$,
J.~Dolejsi$^{\rm 129}$,
Z.~Dolezal$^{\rm 129}$,
B.A.~Dolgoshein$^{\rm 98}$$^{,*}$,
M.~Donadelli$^{\rm 24d}$,
S.~Donati$^{\rm 124a,124b}$,
P.~Dondero$^{\rm 121a,121b}$,
J.~Donini$^{\rm 34}$,
J.~Dopke$^{\rm 131}$,
A.~Doria$^{\rm 104a}$,
M.T.~Dova$^{\rm 71}$,
A.T.~Doyle$^{\rm 53}$,
M.~Dris$^{\rm 10}$,
E.~Dubreuil$^{\rm 34}$,
E.~Duchovni$^{\rm 173}$,
G.~Duckeck$^{\rm 100}$,
O.A.~Ducu$^{\rm 26a,85}$,
D.~Duda$^{\rm 176}$,
A.~Dudarev$^{\rm 30}$,
L.~Duflot$^{\rm 117}$,
L.~Duguid$^{\rm 77}$,
M.~D\"uhrssen$^{\rm 30}$,
M.~Dunford$^{\rm 58a}$,
H.~Duran~Yildiz$^{\rm 4a}$,
M.~D\"uren$^{\rm 52}$,
A.~Durglishvili$^{\rm 51b}$,
D.~Duschinger$^{\rm 44}$,
M.~Dwuznik$^{\rm 38a}$,
M.~Dyndal$^{\rm 38a}$,
W.~Edson$^{\rm 2}$,
N.C.~Edwards$^{\rm 46}$,
W.~Ehrenfeld$^{\rm 21}$,
T.~Eifert$^{\rm 30}$,
G.~Eigen$^{\rm 14}$,
K.~Einsweiler$^{\rm 15}$,
T.~Ekelof$^{\rm 167}$,
M.~El~Kacimi$^{\rm 136c}$,
M.~Ellert$^{\rm 167}$,
S.~Elles$^{\rm 5}$,
F.~Ellinghaus$^{\rm 83}$,
A.A.~Elliot$^{\rm 170}$,
N.~Ellis$^{\rm 30}$,
J.~Elmsheuser$^{\rm 100}$,
M.~Elsing$^{\rm 30}$,
D.~Emeliyanov$^{\rm 131}$,
Y.~Enari$^{\rm 156}$,
O.C.~Endner$^{\rm 83}$,
M.~Endo$^{\rm 118}$,
R.~Engelmann$^{\rm 149}$,
J.~Erdmann$^{\rm 43}$,
A.~Ereditato$^{\rm 17}$,
D.~Eriksson$^{\rm 147a}$,
G.~Ernis$^{\rm 176}$,
J.~Ernst$^{\rm 2}$,
M.~Ernst$^{\rm 25}$,
S.~Errede$^{\rm 166}$,
E.~Ertel$^{\rm 83}$,
M.~Escalier$^{\rm 117}$,
H.~Esch$^{\rm 43}$,
C.~Escobar$^{\rm 125}$,
B.~Esposito$^{\rm 47}$,
A.I.~Etienvre$^{\rm 137}$,
E.~Etzion$^{\rm 154}$,
H.~Evans$^{\rm 61}$,
A.~Ezhilov$^{\rm 123}$,
L.~Fabbri$^{\rm 20a,20b}$,
G.~Facini$^{\rm 31}$,
R.M.~Fakhrutdinov$^{\rm 130}$,
S.~Falciano$^{\rm 133a}$,
R.J.~Falla$^{\rm 78}$,
J.~Faltova$^{\rm 129}$,
Y.~Fang$^{\rm 33a}$,
M.~Fanti$^{\rm 91a,91b}$,
A.~Farbin$^{\rm 8}$,
A.~Farilla$^{\rm 135a}$,
T.~Farooque$^{\rm 12}$,
S.~Farrell$^{\rm 15}$,
S.M.~Farrington$^{\rm 171}$,
P.~Farthouat$^{\rm 30}$,
F.~Fassi$^{\rm 136e}$,
P.~Fassnacht$^{\rm 30}$,
D.~Fassouliotis$^{\rm 9}$,
A.~Favareto$^{\rm 50a,50b}$,
L.~Fayard$^{\rm 117}$,
P.~Federic$^{\rm 145a}$,
O.L.~Fedin$^{\rm 123}$$^{,l}$,
W.~Fedorko$^{\rm 169}$,
S.~Feigl$^{\rm 30}$,
L.~Feligioni$^{\rm 85}$,
C.~Feng$^{\rm 33d}$,
E.J.~Feng$^{\rm 6}$,
H.~Feng$^{\rm 89}$,
A.B.~Fenyuk$^{\rm 130}$,
P.~Fernandez~Martinez$^{\rm 168}$,
S.~Fernandez~Perez$^{\rm 30}$,
S.~Ferrag$^{\rm 53}$,
J.~Ferrando$^{\rm 53}$,
A.~Ferrari$^{\rm 167}$,
P.~Ferrari$^{\rm 107}$,
R.~Ferrari$^{\rm 121a}$,
D.E.~Ferreira~de~Lima$^{\rm 53}$,
A.~Ferrer$^{\rm 168}$,
D.~Ferrere$^{\rm 49}$,
C.~Ferretti$^{\rm 89}$,
A.~Ferretto~Parodi$^{\rm 50a,50b}$,
M.~Fiascaris$^{\rm 31}$,
F.~Fiedler$^{\rm 83}$,
A.~Filip\v{c}i\v{c}$^{\rm 75}$,
M.~Filipuzzi$^{\rm 42}$,
F.~Filthaut$^{\rm 106}$,
M.~Fincke-Keeler$^{\rm 170}$,
K.D.~Finelli$^{\rm 151}$,
M.C.N.~Fiolhais$^{\rm 126a,126c}$,
L.~Fiorini$^{\rm 168}$,
A.~Firan$^{\rm 40}$,
A.~Fischer$^{\rm 2}$,
C.~Fischer$^{\rm 12}$,
J.~Fischer$^{\rm 176}$,
W.C.~Fisher$^{\rm 90}$,
E.A.~Fitzgerald$^{\rm 23}$,
M.~Flechl$^{\rm 48}$,
I.~Fleck$^{\rm 142}$,
P.~Fleischmann$^{\rm 89}$,
S.~Fleischmann$^{\rm 176}$,
G.T.~Fletcher$^{\rm 140}$,
G.~Fletcher$^{\rm 76}$,
T.~Flick$^{\rm 176}$,
A.~Floderus$^{\rm 81}$,
L.R.~Flores~Castillo$^{\rm 60a}$,
M.J.~Flowerdew$^{\rm 101}$,
A.~Formica$^{\rm 137}$,
A.~Forti$^{\rm 84}$,
D.~Fournier$^{\rm 117}$,
H.~Fox$^{\rm 72}$,
S.~Fracchia$^{\rm 12}$,
P.~Francavilla$^{\rm 80}$,
M.~Franchini$^{\rm 20a,20b}$,
D.~Francis$^{\rm 30}$,
L.~Franconi$^{\rm 119}$,
M.~Franklin$^{\rm 57}$,
M.~Fraternali$^{\rm 121a,121b}$,
D.~Freeborn$^{\rm 78}$,
S.T.~French$^{\rm 28}$,
F.~Friedrich$^{\rm 44}$,
D.~Froidevaux$^{\rm 30}$,
J.A.~Frost$^{\rm 120}$,
C.~Fukunaga$^{\rm 157}$,
E.~Fullana~Torregrosa$^{\rm 83}$,
B.G.~Fulsom$^{\rm 144}$,
J.~Fuster$^{\rm 168}$,
C.~Gabaldon$^{\rm 55}$,
O.~Gabizon$^{\rm 176}$,
A.~Gabrielli$^{\rm 20a,20b}$,
A.~Gabrielli$^{\rm 133a,133b}$,
S.~Gadatsch$^{\rm 107}$,
S.~Gadomski$^{\rm 49}$,
G.~Gagliardi$^{\rm 50a,50b}$,
P.~Gagnon$^{\rm 61}$,
C.~Galea$^{\rm 106}$,
B.~Galhardo$^{\rm 126a,126c}$,
E.J.~Gallas$^{\rm 120}$,
B.J.~Gallop$^{\rm 131}$,
P.~Gallus$^{\rm 128}$,
G.~Galster$^{\rm 36}$,
K.K.~Gan$^{\rm 111}$,
J.~Gao$^{\rm 33b,85}$,
Y.~Gao$^{\rm 46}$,
Y.S.~Gao$^{\rm 144}$$^{,e}$,
F.M.~Garay~Walls$^{\rm 46}$,
F.~Garberson$^{\rm 177}$,
C.~Garc\'ia$^{\rm 168}$,
J.E.~Garc\'ia~Navarro$^{\rm 168}$,
M.~Garcia-Sciveres$^{\rm 15}$,
R.W.~Gardner$^{\rm 31}$,
N.~Garelli$^{\rm 144}$,
V.~Garonne$^{\rm 30}$,
C.~Gatti$^{\rm 47}$,
G.~Gaudio$^{\rm 121a}$,
B.~Gaur$^{\rm 142}$,
L.~Gauthier$^{\rm 95}$,
P.~Gauzzi$^{\rm 133a,133b}$,
I.L.~Gavrilenko$^{\rm 96}$,
C.~Gay$^{\rm 169}$,
G.~Gaycken$^{\rm 21}$,
E.N.~Gazis$^{\rm 10}$,
P.~Ge$^{\rm 33d}$,
Z.~Gecse$^{\rm 169}$,
C.N.P.~Gee$^{\rm 131}$,
D.A.A.~Geerts$^{\rm 107}$,
Ch.~Geich-Gimbel$^{\rm 21}$,
C.~Gemme$^{\rm 50a}$,
M.H.~Genest$^{\rm 55}$,
S.~Gentile$^{\rm 133a,133b}$,
M.~George$^{\rm 54}$,
S.~George$^{\rm 77}$,
D.~Gerbaudo$^{\rm 164}$,
A.~Gershon$^{\rm 154}$,
H.~Ghazlane$^{\rm 136b}$,
N.~Ghodbane$^{\rm 34}$,
B.~Giacobbe$^{\rm 20a}$,
S.~Giagu$^{\rm 133a,133b}$,
V.~Giangiobbe$^{\rm 12}$,
P.~Giannetti$^{\rm 124a,124b}$,
F.~Gianotti$^{\rm 30}$,
B.~Gibbard$^{\rm 25}$,
S.M.~Gibson$^{\rm 77}$,
M.~Gilchriese$^{\rm 15}$,
T.P.S.~Gillam$^{\rm 28}$,
D.~Gillberg$^{\rm 30}$,
G.~Gilles$^{\rm 34}$,
D.M.~Gingrich$^{\rm 3}$$^{,d}$,
N.~Giokaris$^{\rm 9}$,
M.P.~Giordani$^{\rm 165a,165c}$,
F.M.~Giorgi$^{\rm 20a}$,
F.M.~Giorgi$^{\rm 16}$,
P.F.~Giraud$^{\rm 137}$,
P.~Giromini$^{\rm 47}$,
D.~Giugni$^{\rm 91a}$,
C.~Giuliani$^{\rm 48}$,
M.~Giulini$^{\rm 58b}$,
B.K.~Gjelsten$^{\rm 119}$,
S.~Gkaitatzis$^{\rm 155}$,
I.~Gkialas$^{\rm 155}$,
E.L.~Gkougkousis$^{\rm 117}$,
L.K.~Gladilin$^{\rm 99}$,
C.~Glasman$^{\rm 82}$,
J.~Glatzer$^{\rm 30}$,
P.C.F.~Glaysher$^{\rm 46}$,
A.~Glazov$^{\rm 42}$,
M.~Goblirsch-Kolb$^{\rm 101}$,
J.R.~Goddard$^{\rm 76}$,
J.~Godlewski$^{\rm 39}$,
S.~Goldfarb$^{\rm 89}$,
T.~Golling$^{\rm 49}$,
D.~Golubkov$^{\rm 130}$,
A.~Gomes$^{\rm 126a,126b,126d}$,
R.~Gon\c{c}alo$^{\rm 126a}$,
J.~Goncalves~Pinto~Firmino~Da~Costa$^{\rm 137}$,
L.~Gonella$^{\rm 21}$,
S.~Gonz\'alez~de~la~Hoz$^{\rm 168}$,
G.~Gonzalez~Parra$^{\rm 12}$,
S.~Gonzalez-Sevilla$^{\rm 49}$,
L.~Goossens$^{\rm 30}$,
P.A.~Gorbounov$^{\rm 97}$,
H.A.~Gordon$^{\rm 25}$,
I.~Gorelov$^{\rm 105}$,
B.~Gorini$^{\rm 30}$,
E.~Gorini$^{\rm 73a,73b}$,
A.~Gori\v{s}ek$^{\rm 75}$,
E.~Gornicki$^{\rm 39}$,
A.T.~Goshaw$^{\rm 45}$,
C.~G\"ossling$^{\rm 43}$,
M.I.~Gostkin$^{\rm 65}$,
D.~Goujdami$^{\rm 136c}$,
A.G.~Goussiou$^{\rm 139}$,
H.M.X.~Grabas$^{\rm 138}$,
L.~Graber$^{\rm 54}$,
I.~Grabowska-Bold$^{\rm 38a}$,
P.~Grafstr\"om$^{\rm 20a,20b}$,
K-J.~Grahn$^{\rm 42}$,
J.~Gramling$^{\rm 49}$,
E.~Gramstad$^{\rm 119}$,
S.~Grancagnolo$^{\rm 16}$,
V.~Grassi$^{\rm 149}$,
V.~Gratchev$^{\rm 123}$,
H.M.~Gray$^{\rm 30}$,
E.~Graziani$^{\rm 135a}$,
Z.D.~Greenwood$^{\rm 79}$$^{,m}$,
K.~Gregersen$^{\rm 78}$,
I.M.~Gregor$^{\rm 42}$,
P.~Grenier$^{\rm 144}$,
J.~Griffiths$^{\rm 8}$,
A.A.~Grillo$^{\rm 138}$,
K.~Grimm$^{\rm 72}$,
S.~Grinstein$^{\rm 12}$$^{,n}$,
Ph.~Gris$^{\rm 34}$,
Y.V.~Grishkevich$^{\rm 99}$,
J.-F.~Grivaz$^{\rm 117}$,
J.P.~Grohs$^{\rm 44}$,
A.~Grohsjean$^{\rm 42}$,
E.~Gross$^{\rm 173}$,
J.~Grosse-Knetter$^{\rm 54}$,
G.C.~Grossi$^{\rm 134a,134b}$,
Z.J.~Grout$^{\rm 150}$,
L.~Guan$^{\rm 33b}$,
J.~Guenther$^{\rm 128}$,
F.~Guescini$^{\rm 49}$,
D.~Guest$^{\rm 177}$,
O.~Gueta$^{\rm 154}$,
E.~Guido$^{\rm 50a,50b}$,
T.~Guillemin$^{\rm 117}$,
S.~Guindon$^{\rm 2}$,
U.~Gul$^{\rm 53}$,
C.~Gumpert$^{\rm 44}$,
J.~Guo$^{\rm 33e}$,
S.~Gupta$^{\rm 120}$,
P.~Gutierrez$^{\rm 113}$,
N.G.~Gutierrez~Ortiz$^{\rm 53}$,
C.~Gutschow$^{\rm 44}$,
C.~Guyot$^{\rm 137}$,
C.~Gwenlan$^{\rm 120}$,
C.B.~Gwilliam$^{\rm 74}$,
A.~Haas$^{\rm 110}$,
C.~Haber$^{\rm 15}$,
H.K.~Hadavand$^{\rm 8}$,
N.~Haddad$^{\rm 136e}$,
P.~Haefner$^{\rm 21}$,
S.~Hageb\"ock$^{\rm 21}$,
Z.~Hajduk$^{\rm 39}$,
H.~Hakobyan$^{\rm 178}$,
M.~Haleem$^{\rm 42}$,
J.~Haley$^{\rm 114}$,
D.~Hall$^{\rm 120}$,
G.~Halladjian$^{\rm 90}$,
G.D.~Hallewell$^{\rm 85}$,
K.~Hamacher$^{\rm 176}$,
P.~Hamal$^{\rm 115}$,
K.~Hamano$^{\rm 170}$,
M.~Hamer$^{\rm 54}$,
A.~Hamilton$^{\rm 146a}$,
S.~Hamilton$^{\rm 162}$,
G.N.~Hamity$^{\rm 146c}$,
P.G.~Hamnett$^{\rm 42}$,
L.~Han$^{\rm 33b}$,
K.~Hanagaki$^{\rm 118}$,
K.~Hanawa$^{\rm 156}$,
M.~Hance$^{\rm 15}$,
P.~Hanke$^{\rm 58a}$,
R.~Hanna$^{\rm 137}$,
J.B.~Hansen$^{\rm 36}$,
J.D.~Hansen$^{\rm 36}$,
P.H.~Hansen$^{\rm 36}$,
K.~Hara$^{\rm 161}$,
A.S.~Hard$^{\rm 174}$,
T.~Harenberg$^{\rm 176}$,
F.~Hariri$^{\rm 117}$,
S.~Harkusha$^{\rm 92}$,
R.D.~Harrington$^{\rm 46}$,
P.F.~Harrison$^{\rm 171}$,
F.~Hartjes$^{\rm 107}$,
M.~Hasegawa$^{\rm 67}$,
S.~Hasegawa$^{\rm 103}$,
Y.~Hasegawa$^{\rm 141}$,
A.~Hasib$^{\rm 113}$,
S.~Hassani$^{\rm 137}$,
S.~Haug$^{\rm 17}$,
R.~Hauser$^{\rm 90}$,
L.~Hauswald$^{\rm 44}$,
M.~Havranek$^{\rm 127}$,
C.M.~Hawkes$^{\rm 18}$,
R.J.~Hawkings$^{\rm 30}$,
A.D.~Hawkins$^{\rm 81}$,
T.~Hayashi$^{\rm 161}$,
D.~Hayden$^{\rm 90}$,
C.P.~Hays$^{\rm 120}$,
J.M.~Hays$^{\rm 76}$,
H.S.~Hayward$^{\rm 74}$,
S.J.~Haywood$^{\rm 131}$,
S.J.~Head$^{\rm 18}$,
T.~Heck$^{\rm 83}$,
V.~Hedberg$^{\rm 81}$,
L.~Heelan$^{\rm 8}$,
S.~Heim$^{\rm 122}$,
T.~Heim$^{\rm 176}$,
B.~Heinemann$^{\rm 15}$,
L.~Heinrich$^{\rm 110}$,
J.~Hejbal$^{\rm 127}$,
L.~Helary$^{\rm 22}$,
S.~Hellman$^{\rm 147a,147b}$,
D.~Hellmich$^{\rm 21}$,
C.~Helsens$^{\rm 30}$,
J.~Henderson$^{\rm 120}$,
R.C.W.~Henderson$^{\rm 72}$,
Y.~Heng$^{\rm 174}$,
C.~Hengler$^{\rm 42}$,
A.~Henrichs$^{\rm 177}$,
A.M.~Henriques~Correia$^{\rm 30}$,
S.~Henrot-Versille$^{\rm 117}$,
G.H.~Herbert$^{\rm 16}$,
Y.~Hern\'andez~Jim\'enez$^{\rm 168}$,
R.~Herrberg-Schubert$^{\rm 16}$,
G.~Herten$^{\rm 48}$,
R.~Hertenberger$^{\rm 100}$,
L.~Hervas$^{\rm 30}$,
G.G.~Hesketh$^{\rm 78}$,
N.P.~Hessey$^{\rm 107}$,
J.W.~Hetherly$^{\rm 40}$,
R.~Hickling$^{\rm 76}$,
E.~Hig\'on-Rodriguez$^{\rm 168}$,
E.~Hill$^{\rm 170}$,
J.C.~Hill$^{\rm 28}$,
K.H.~Hiller$^{\rm 42}$,
S.J.~Hillier$^{\rm 18}$,
I.~Hinchliffe$^{\rm 15}$,
E.~Hines$^{\rm 122}$,
R.R.~Hinman$^{\rm 15}$,
M.~Hirose$^{\rm 158}$,
D.~Hirschbuehl$^{\rm 176}$,
J.~Hobbs$^{\rm 149}$,
N.~Hod$^{\rm 107}$,
M.C.~Hodgkinson$^{\rm 140}$,
P.~Hodgson$^{\rm 140}$,
A.~Hoecker$^{\rm 30}$,
M.R.~Hoeferkamp$^{\rm 105}$,
F.~Hoenig$^{\rm 100}$,
M.~Hohlfeld$^{\rm 83}$,
D.~Hohn$^{\rm 21}$,
T.R.~Holmes$^{\rm 15}$,
T.M.~Hong$^{\rm 122}$,
L.~Hooft~van~Huysduynen$^{\rm 110}$,
W.H.~Hopkins$^{\rm 116}$,
Y.~Horii$^{\rm 103}$,
A.J.~Horton$^{\rm 143}$,
J-Y.~Hostachy$^{\rm 55}$,
S.~Hou$^{\rm 152}$,
A.~Hoummada$^{\rm 136a}$,
J.~Howard$^{\rm 120}$,
J.~Howarth$^{\rm 42}$,
M.~Hrabovsky$^{\rm 115}$,
I.~Hristova$^{\rm 16}$,
J.~Hrivnac$^{\rm 117}$,
T.~Hryn'ova$^{\rm 5}$,
A.~Hrynevich$^{\rm 93}$,
C.~Hsu$^{\rm 146c}$,
P.J.~Hsu$^{\rm 152}$$^{,o}$,
S.-C.~Hsu$^{\rm 139}$,
D.~Hu$^{\rm 35}$,
Q.~Hu$^{\rm 33b}$,
X.~Hu$^{\rm 89}$,
Y.~Huang$^{\rm 42}$,
Z.~Hubacek$^{\rm 30}$,
F.~Hubaut$^{\rm 85}$,
F.~Huegging$^{\rm 21}$,
T.B.~Huffman$^{\rm 120}$,
E.W.~Hughes$^{\rm 35}$,
G.~Hughes$^{\rm 72}$,
M.~Huhtinen$^{\rm 30}$,
T.A.~H\"ulsing$^{\rm 83}$,
N.~Huseynov$^{\rm 65}$$^{,b}$,
J.~Huston$^{\rm 90}$,
J.~Huth$^{\rm 57}$,
G.~Iacobucci$^{\rm 49}$,
G.~Iakovidis$^{\rm 25}$,
I.~Ibragimov$^{\rm 142}$,
L.~Iconomidou-Fayard$^{\rm 117}$,
E.~Ideal$^{\rm 177}$,
Z.~Idrissi$^{\rm 136e}$,
P.~Iengo$^{\rm 104a}$,
O.~Igonkina$^{\rm 107}$,
T.~Iizawa$^{\rm 172}$,
Y.~Ikegami$^{\rm 66}$,
K.~Ikematsu$^{\rm 142}$,
M.~Ikeno$^{\rm 66}$,
Y.~Ilchenko$^{\rm 31}$$^{,p}$,
D.~Iliadis$^{\rm 155}$,
N.~Ilic$^{\rm 159}$,
Y.~Inamaru$^{\rm 67}$,
T.~Ince$^{\rm 101}$,
P.~Ioannou$^{\rm 9}$,
M.~Iodice$^{\rm 135a}$,
K.~Iordanidou$^{\rm 9}$,
V.~Ippolito$^{\rm 57}$,
A.~Irles~Quiles$^{\rm 168}$,
C.~Isaksson$^{\rm 167}$,
M.~Ishino$^{\rm 68}$,
M.~Ishitsuka$^{\rm 158}$,
R.~Ishmukhametov$^{\rm 111}$,
C.~Issever$^{\rm 120}$,
S.~Istin$^{\rm 19a}$,
J.M.~Iturbe~Ponce$^{\rm 84}$,
R.~Iuppa$^{\rm 134a,134b}$,
J.~Ivarsson$^{\rm 81}$,
W.~Iwanski$^{\rm 39}$,
H.~Iwasaki$^{\rm 66}$,
J.M.~Izen$^{\rm 41}$,
V.~Izzo$^{\rm 104a}$,
S.~Jabbar$^{\rm 3}$,
B.~Jackson$^{\rm 122}$,
M.~Jackson$^{\rm 74}$,
P.~Jackson$^{\rm 1}$,
M.R.~Jaekel$^{\rm 30}$,
V.~Jain$^{\rm 2}$,
K.~Jakobs$^{\rm 48}$,
S.~Jakobsen$^{\rm 30}$,
T.~Jakoubek$^{\rm 127}$,
J.~Jakubek$^{\rm 128}$,
D.O.~Jamin$^{\rm 152}$,
D.K.~Jana$^{\rm 79}$,
E.~Jansen$^{\rm 78}$,
R.W.~Jansky$^{\rm 62}$,
J.~Janssen$^{\rm 21}$,
M.~Janus$^{\rm 171}$,
G.~Jarlskog$^{\rm 81}$,
N.~Javadov$^{\rm 65}$$^{,b}$,
T.~Jav\r{u}rek$^{\rm 48}$,
L.~Jeanty$^{\rm 15}$,
J.~Jejelava$^{\rm 51a}$$^{,q}$,
G.-Y.~Jeng$^{\rm 151}$,
D.~Jennens$^{\rm 88}$,
P.~Jenni$^{\rm 48}$$^{,r}$,
J.~Jentzsch$^{\rm 43}$,
C.~Jeske$^{\rm 171}$,
S.~J\'ez\'equel$^{\rm 5}$,
H.~Ji$^{\rm 174}$,
J.~Jia$^{\rm 149}$,
Y.~Jiang$^{\rm 33b}$,
J.~Jimenez~Pena$^{\rm 168}$,
S.~Jin$^{\rm 33a}$,
A.~Jinaru$^{\rm 26a}$,
O.~Jinnouchi$^{\rm 158}$,
M.D.~Joergensen$^{\rm 36}$,
P.~Johansson$^{\rm 140}$,
K.A.~Johns$^{\rm 7}$,
K.~Jon-And$^{\rm 147a,147b}$,
G.~Jones$^{\rm 171}$,
R.W.L.~Jones$^{\rm 72}$,
T.J.~Jones$^{\rm 74}$,
J.~Jongmanns$^{\rm 58a}$,
P.M.~Jorge$^{\rm 126a,126b}$,
K.D.~Joshi$^{\rm 84}$,
J.~Jovicevic$^{\rm 160a}$,
X.~Ju$^{\rm 174}$,
C.A.~Jung$^{\rm 43}$,
P.~Jussel$^{\rm 62}$,
A.~Juste~Rozas$^{\rm 12}$$^{,n}$,
M.~Kaci$^{\rm 168}$,
A.~Kaczmarska$^{\rm 39}$,
M.~Kado$^{\rm 117}$,
H.~Kagan$^{\rm 111}$,
M.~Kagan$^{\rm 144}$,
S.J.~Kahn$^{\rm 85}$,
E.~Kajomovitz$^{\rm 45}$,
C.W.~Kalderon$^{\rm 120}$,
S.~Kama$^{\rm 40}$,
A.~Kamenshchikov$^{\rm 130}$,
N.~Kanaya$^{\rm 156}$,
M.~Kaneda$^{\rm 30}$,
S.~Kaneti$^{\rm 28}$,
V.A.~Kantserov$^{\rm 98}$,
J.~Kanzaki$^{\rm 66}$,
B.~Kaplan$^{\rm 110}$,
A.~Kapliy$^{\rm 31}$,
D.~Kar$^{\rm 53}$,
K.~Karakostas$^{\rm 10}$,
A.~Karamaoun$^{\rm 3}$,
N.~Karastathis$^{\rm 10,107}$,
M.J.~Kareem$^{\rm 54}$,
M.~Karnevskiy$^{\rm 83}$,
S.N.~Karpov$^{\rm 65}$,
Z.M.~Karpova$^{\rm 65}$,
K.~Karthik$^{\rm 110}$,
V.~Kartvelishvili$^{\rm 72}$,
A.N.~Karyukhin$^{\rm 130}$,
L.~Kashif$^{\rm 174}$,
R.D.~Kass$^{\rm 111}$,
A.~Kastanas$^{\rm 14}$,
Y.~Kataoka$^{\rm 156}$,
A.~Katre$^{\rm 49}$,
J.~Katzy$^{\rm 42}$,
K.~Kawagoe$^{\rm 70}$,
T.~Kawamoto$^{\rm 156}$,
G.~Kawamura$^{\rm 54}$,
S.~Kazama$^{\rm 156}$,
V.F.~Kazanin$^{\rm 109}$,
M.Y.~Kazarinov$^{\rm 65}$,
R.~Keeler$^{\rm 170}$,
R.~Kehoe$^{\rm 40}$,
M.~Keil$^{\rm 54}$,
J.S.~Keller$^{\rm 42}$,
J.J.~Kempster$^{\rm 77}$,
H.~Keoshkerian$^{\rm 84}$,
O.~Kepka$^{\rm 127}$,
B.P.~Ker\v{s}evan$^{\rm 75}$,
S.~Kersten$^{\rm 176}$,
R.A.~Keyes$^{\rm 87}$,
F.~Khalil-zada$^{\rm 11}$,
H.~Khandanyan$^{\rm 147a,147b}$,
A.~Khanov$^{\rm 114}$,
A.~Kharlamov$^{\rm 109}$,
T.J.~Khoo$^{\rm 28}$,
G.~Khoriauli$^{\rm 21}$,
V.~Khovanskiy$^{\rm 97}$,
E.~Khramov$^{\rm 65}$,
J.~Khubua$^{\rm 51b}$$^{,s}$,
H.Y.~Kim$^{\rm 8}$,
H.~Kim$^{\rm 147a,147b}$,
S.H.~Kim$^{\rm 161}$,
Y.~Kim$^{\rm 31}$,
N.~Kimura$^{\rm 155}$,
O.M.~Kind$^{\rm 16}$,
B.T.~King$^{\rm 74}$,
M.~King$^{\rm 168}$,
R.S.B.~King$^{\rm 120}$,
S.B.~King$^{\rm 169}$,
J.~Kirk$^{\rm 131}$,
A.E.~Kiryunin$^{\rm 101}$,
T.~Kishimoto$^{\rm 67}$,
D.~Kisielewska$^{\rm 38a}$,
F.~Kiss$^{\rm 48}$,
K.~Kiuchi$^{\rm 161}$,
E.~Kladiva$^{\rm 145b}$,
M.H.~Klein$^{\rm 35}$,
M.~Klein$^{\rm 74}$,
U.~Klein$^{\rm 74}$,
K.~Kleinknecht$^{\rm 83}$,
P.~Klimek$^{\rm 147a,147b}$,
A.~Klimentov$^{\rm 25}$,
R.~Klingenberg$^{\rm 43}$,
J.A.~Klinger$^{\rm 84}$,
T.~Klioutchnikova$^{\rm 30}$,
P.F.~Klok$^{\rm 106}$,
E.-E.~Kluge$^{\rm 58a}$,
P.~Kluit$^{\rm 107}$,
S.~Kluth$^{\rm 101}$,
E.~Kneringer$^{\rm 62}$,
E.B.F.G.~Knoops$^{\rm 85}$,
A.~Knue$^{\rm 53}$,
D.~Kobayashi$^{\rm 158}$,
T.~Kobayashi$^{\rm 156}$,
M.~Kobel$^{\rm 44}$,
M.~Kocian$^{\rm 144}$,
P.~Kodys$^{\rm 129}$,
T.~Koffas$^{\rm 29}$,
E.~Koffeman$^{\rm 107}$,
L.A.~Kogan$^{\rm 120}$,
S.~Kohlmann$^{\rm 176}$,
Z.~Kohout$^{\rm 128}$,
T.~Kohriki$^{\rm 66}$,
T.~Koi$^{\rm 144}$,
H.~Kolanoski$^{\rm 16}$,
I.~Koletsou$^{\rm 5}$,
A.A.~Komar$^{\rm 96}$$^{,*}$,
Y.~Komori$^{\rm 156}$,
T.~Kondo$^{\rm 66}$,
N.~Kondrashova$^{\rm 42}$,
K.~K\"oneke$^{\rm 48}$,
A.C.~K\"onig$^{\rm 106}$,
S.~K\"onig$^{\rm 83}$,
T.~Kono$^{\rm 66}$$^{,t}$,
R.~Konoplich$^{\rm 110}$$^{,u}$,
N.~Konstantinidis$^{\rm 78}$,
R.~Kopeliansky$^{\rm 153}$,
S.~Koperny$^{\rm 38a}$,
L.~K\"opke$^{\rm 83}$,
A.K.~Kopp$^{\rm 48}$,
K.~Korcyl$^{\rm 39}$,
K.~Kordas$^{\rm 155}$,
A.~Korn$^{\rm 78}$,
A.A.~Korol$^{\rm 109}$$^{,c}$,
I.~Korolkov$^{\rm 12}$,
E.V.~Korolkova$^{\rm 140}$,
O.~Kortner$^{\rm 101}$,
S.~Kortner$^{\rm 101}$,
T.~Kosek$^{\rm 129}$,
V.V.~Kostyukhin$^{\rm 21}$,
V.M.~Kotov$^{\rm 65}$,
A.~Kotwal$^{\rm 45}$,
A.~Kourkoumeli-Charalampidi$^{\rm 155}$,
C.~Kourkoumelis$^{\rm 9}$,
V.~Kouskoura$^{\rm 25}$,
A.~Koutsman$^{\rm 160a}$,
R.~Kowalewski$^{\rm 170}$,
T.Z.~Kowalski$^{\rm 38a}$,
W.~Kozanecki$^{\rm 137}$,
A.S.~Kozhin$^{\rm 130}$,
V.A.~Kramarenko$^{\rm 99}$,
G.~Kramberger$^{\rm 75}$,
D.~Krasnopevtsev$^{\rm 98}$,
M.W.~Krasny$^{\rm 80}$,
A.~Krasznahorkay$^{\rm 30}$,
J.K.~Kraus$^{\rm 21}$,
A.~Kravchenko$^{\rm 25}$,
S.~Kreiss$^{\rm 110}$,
M.~Kretz$^{\rm 58c}$,
J.~Kretzschmar$^{\rm 74}$,
K.~Kreutzfeldt$^{\rm 52}$,
P.~Krieger$^{\rm 159}$,
K.~Krizka$^{\rm 31}$,
K.~Kroeninger$^{\rm 43}$,
H.~Kroha$^{\rm 101}$,
J.~Kroll$^{\rm 122}$,
J.~Kroseberg$^{\rm 21}$,
J.~Krstic$^{\rm 13}$,
U.~Kruchonak$^{\rm 65}$,
H.~Kr\"uger$^{\rm 21}$,
N.~Krumnack$^{\rm 64}$,
Z.V.~Krumshteyn$^{\rm 65}$,
A.~Kruse$^{\rm 174}$,
M.C.~Kruse$^{\rm 45}$,
M.~Kruskal$^{\rm 22}$,
T.~Kubota$^{\rm 88}$,
H.~Kucuk$^{\rm 78}$,
S.~Kuday$^{\rm 4c}$,
S.~Kuehn$^{\rm 48}$,
A.~Kugel$^{\rm 58c}$,
F.~Kuger$^{\rm 175}$,
A.~Kuhl$^{\rm 138}$,
T.~Kuhl$^{\rm 42}$,
V.~Kukhtin$^{\rm 65}$,
Y.~Kulchitsky$^{\rm 92}$,
S.~Kuleshov$^{\rm 32b}$,
M.~Kuna$^{\rm 133a,133b}$,
T.~Kunigo$^{\rm 68}$,
A.~Kupco$^{\rm 127}$,
H.~Kurashige$^{\rm 67}$,
Y.A.~Kurochkin$^{\rm 92}$,
R.~Kurumida$^{\rm 67}$,
V.~Kus$^{\rm 127}$,
E.S.~Kuwertz$^{\rm 148}$,
M.~Kuze$^{\rm 158}$,
J.~Kvita$^{\rm 115}$,
T.~Kwan$^{\rm 170}$,
D.~Kyriazopoulos$^{\rm 140}$,
A.~La~Rosa$^{\rm 49}$,
J.L.~La~Rosa~Navarro$^{\rm 24d}$,
L.~La~Rotonda$^{\rm 37a,37b}$,
C.~Lacasta$^{\rm 168}$,
F.~Lacava$^{\rm 133a,133b}$,
J.~Lacey$^{\rm 29}$,
H.~Lacker$^{\rm 16}$,
D.~Lacour$^{\rm 80}$,
V.R.~Lacuesta$^{\rm 168}$,
E.~Ladygin$^{\rm 65}$,
R.~Lafaye$^{\rm 5}$,
B.~Laforge$^{\rm 80}$,
T.~Lagouri$^{\rm 177}$,
S.~Lai$^{\rm 48}$,
L.~Lambourne$^{\rm 78}$,
S.~Lammers$^{\rm 61}$,
C.L.~Lampen$^{\rm 7}$,
W.~Lampl$^{\rm 7}$,
E.~Lan\c{c}on$^{\rm 137}$,
U.~Landgraf$^{\rm 48}$,
M.P.J.~Landon$^{\rm 76}$,
V.S.~Lang$^{\rm 58a}$,
A.J.~Lankford$^{\rm 164}$,
F.~Lanni$^{\rm 25}$,
K.~Lantzsch$^{\rm 30}$,
S.~Laplace$^{\rm 80}$,
C.~Lapoire$^{\rm 30}$,
J.F.~Laporte$^{\rm 137}$,
T.~Lari$^{\rm 91a}$,
F.~Lasagni~Manghi$^{\rm 20a,20b}$,
M.~Lassnig$^{\rm 30}$,
P.~Laurelli$^{\rm 47}$,
W.~Lavrijsen$^{\rm 15}$,
A.T.~Law$^{\rm 138}$,
P.~Laycock$^{\rm 74}$,
O.~Le~Dortz$^{\rm 80}$,
E.~Le~Guirriec$^{\rm 85}$,
E.~Le~Menedeu$^{\rm 12}$,
T.~LeCompte$^{\rm 6}$,
F.~Ledroit-Guillon$^{\rm 55}$,
C.A.~Lee$^{\rm 146b}$,
S.C.~Lee$^{\rm 152}$,
L.~Lee$^{\rm 1}$,
G.~Lefebvre$^{\rm 80}$,
M.~Lefebvre$^{\rm 170}$,
F.~Legger$^{\rm 100}$,
C.~Leggett$^{\rm 15}$,
A.~Lehan$^{\rm 74}$,
G.~Lehmann~Miotto$^{\rm 30}$,
X.~Lei$^{\rm 7}$,
W.A.~Leight$^{\rm 29}$,
A.~Leisos$^{\rm 155}$,
A.G.~Leister$^{\rm 177}$,
M.A.L.~Leite$^{\rm 24d}$,
R.~Leitner$^{\rm 129}$,
D.~Lellouch$^{\rm 173}$,
B.~Lemmer$^{\rm 54}$,
K.J.C.~Leney$^{\rm 78}$,
T.~Lenz$^{\rm 21}$,
G.~Lenzen$^{\rm 176}$,
B.~Lenzi$^{\rm 30}$,
R.~Leone$^{\rm 7}$,
S.~Leone$^{\rm 124a,124b}$,
C.~Leonidopoulos$^{\rm 46}$,
S.~Leontsinis$^{\rm 10}$,
C.~Leroy$^{\rm 95}$,
C.G.~Lester$^{\rm 28}$,
M.~Levchenko$^{\rm 123}$,
J.~Lev\^eque$^{\rm 5}$,
D.~Levin$^{\rm 89}$,
L.J.~Levinson$^{\rm 173}$,
M.~Levy$^{\rm 18}$,
A.~Lewis$^{\rm 120}$,
A.M.~Leyko$^{\rm 21}$,
M.~Leyton$^{\rm 41}$,
B.~Li$^{\rm 33b}$$^{,v}$,
H.~Li$^{\rm 149}$,
H.L.~Li$^{\rm 31}$,
L.~Li$^{\rm 45}$,
L.~Li$^{\rm 33e}$,
S.~Li$^{\rm 45}$,
Y.~Li$^{\rm 33c}$$^{,w}$,
Z.~Liang$^{\rm 138}$,
H.~Liao$^{\rm 34}$,
B.~Liberti$^{\rm 134a}$,
P.~Lichard$^{\rm 30}$,
K.~Lie$^{\rm 166}$,
J.~Liebal$^{\rm 21}$,
W.~Liebig$^{\rm 14}$,
C.~Limbach$^{\rm 21}$,
A.~Limosani$^{\rm 151}$,
S.C.~Lin$^{\rm 152}$$^{,x}$,
T.H.~Lin$^{\rm 83}$,
F.~Linde$^{\rm 107}$,
B.E.~Lindquist$^{\rm 149}$,
J.T.~Linnemann$^{\rm 90}$,
E.~Lipeles$^{\rm 122}$,
A.~Lipniacka$^{\rm 14}$,
M.~Lisovyi$^{\rm 42}$,
T.M.~Liss$^{\rm 166}$,
D.~Lissauer$^{\rm 25}$,
A.~Lister$^{\rm 169}$,
A.M.~Litke$^{\rm 138}$,
B.~Liu$^{\rm 152}$,
D.~Liu$^{\rm 152}$,
J.~Liu$^{\rm 85}$,
J.B.~Liu$^{\rm 33b}$,
K.~Liu$^{\rm 33b}$$^{,y}$,
L.~Liu$^{\rm 89}$,
M.~Liu$^{\rm 45}$,
M.~Liu$^{\rm 33b}$,
Y.~Liu$^{\rm 33b}$,
M.~Livan$^{\rm 121a,121b}$,
A.~Lleres$^{\rm 55}$,
J.~Llorente~Merino$^{\rm 82}$,
S.L.~Lloyd$^{\rm 76}$,
F.~Lo~Sterzo$^{\rm 152}$,
E.~Lobodzinska$^{\rm 42}$,
P.~Loch$^{\rm 7}$,
W.S.~Lockman$^{\rm 138}$,
F.K.~Loebinger$^{\rm 84}$,
A.E.~Loevschall-Jensen$^{\rm 36}$,
A.~Loginov$^{\rm 177}$,
T.~Lohse$^{\rm 16}$,
K.~Lohwasser$^{\rm 42}$,
M.~Lokajicek$^{\rm 127}$,
B.A.~Long$^{\rm 22}$,
J.D.~Long$^{\rm 89}$,
R.E.~Long$^{\rm 72}$,
K.A.~Looper$^{\rm 111}$,
L.~Lopes$^{\rm 126a}$,
D.~Lopez~Mateos$^{\rm 57}$,
B.~Lopez~Paredes$^{\rm 140}$,
I.~Lopez~Paz$^{\rm 12}$,
J.~Lorenz$^{\rm 100}$,
N.~Lorenzo~Martinez$^{\rm 61}$,
M.~Losada$^{\rm 163}$,
P.~Loscutoff$^{\rm 15}$,
P.J.~L{\"o}sel$^{\rm 100}$,
X.~Lou$^{\rm 33a}$,
A.~Lounis$^{\rm 117}$,
J.~Love$^{\rm 6}$,
P.A.~Love$^{\rm 72}$,
F.~Lu$^{\rm 33a}$,
N.~Lu$^{\rm 89}$,
H.J.~Lubatti$^{\rm 139}$,
C.~Luci$^{\rm 133a,133b}$,
A.~Lucotte$^{\rm 55}$,
F.~Luehring$^{\rm 61}$,
W.~Lukas$^{\rm 62}$,
L.~Luminari$^{\rm 133a}$,
O.~Lundberg$^{\rm 147a,147b}$,
B.~Lund-Jensen$^{\rm 148}$,
M.~Lungwitz$^{\rm 83}$,
D.~Lynn$^{\rm 25}$,
R.~Lysak$^{\rm 127}$,
E.~Lytken$^{\rm 81}$,
H.~Ma$^{\rm 25}$,
L.L.~Ma$^{\rm 33d}$,
G.~Maccarrone$^{\rm 47}$,
A.~Macchiolo$^{\rm 101}$,
C.M.~Macdonald$^{\rm 140}$,
J.~Machado~Miguens$^{\rm 122,126}$,
D.~Macina$^{\rm 30}$,
D.~Madaffari$^{\rm 85}$,
R.~Madar$^{\rm 34}$,
H.J.~Maddocks$^{\rm 72}$,
W.F.~Mader$^{\rm 44}$,
A.~Madsen$^{\rm 167}$,
S.~Maeland$^{\rm 14}$,
T.~Maeno$^{\rm 25}$,
A.~Maevskiy$^{\rm 99}$,
E.~Magradze$^{\rm 54}$,
K.~Mahboubi$^{\rm 48}$,
J.~Mahlstedt$^{\rm 107}$,
C.~Maiani$^{\rm 137}$,
C.~Maidantchik$^{\rm 24a}$,
A.A.~Maier$^{\rm 101}$,
T.~Maier$^{\rm 100}$,
A.~Maio$^{\rm 126a,126b,126d}$,
S.~Majewski$^{\rm 116}$,
Y.~Makida$^{\rm 66}$,
N.~Makovec$^{\rm 117}$,
B.~Malaescu$^{\rm 80}$,
Pa.~Malecki$^{\rm 39}$,
V.P.~Maleev$^{\rm 123}$,
F.~Malek$^{\rm 55}$,
U.~Mallik$^{\rm 63}$,
D.~Malon$^{\rm 6}$,
C.~Malone$^{\rm 144}$,
S.~Maltezos$^{\rm 10}$,
V.M.~Malyshev$^{\rm 109}$,
S.~Malyukov$^{\rm 30}$,
J.~Mamuzic$^{\rm 42}$,
G.~Mancini$^{\rm 47}$,
B.~Mandelli$^{\rm 30}$,
L.~Mandelli$^{\rm 91a}$,
I.~Mandi\'{c}$^{\rm 75}$,
R.~Mandrysch$^{\rm 63}$,
J.~Maneira$^{\rm 126a,126b}$,
A.~Manfredini$^{\rm 101}$,
L.~Manhaes~de~Andrade~Filho$^{\rm 24b}$,
J.~Manjarres~Ramos$^{\rm 160b}$,
A.~Mann$^{\rm 100}$,
P.M.~Manning$^{\rm 138}$,
A.~Manousakis-Katsikakis$^{\rm 9}$,
B.~Mansoulie$^{\rm 137}$,
R.~Mantifel$^{\rm 87}$,
M.~Mantoani$^{\rm 54}$,
L.~Mapelli$^{\rm 30}$,
L.~March$^{\rm 146c}$,
G.~Marchiori$^{\rm 80}$,
M.~Marcisovsky$^{\rm 127}$,
C.P.~Marino$^{\rm 170}$,
M.~Marjanovic$^{\rm 13}$,
F.~Marroquim$^{\rm 24a}$,
S.P.~Marsden$^{\rm 84}$,
Z.~Marshall$^{\rm 15}$,
L.F.~Marti$^{\rm 17}$,
S.~Marti-Garcia$^{\rm 168}$,
B.~Martin$^{\rm 90}$,
T.A.~Martin$^{\rm 171}$,
V.J.~Martin$^{\rm 46}$,
B.~Martin~dit~Latour$^{\rm 14}$,
M.~Martinez$^{\rm 12}$$^{,n}$,
S.~Martin-Haugh$^{\rm 131}$,
V.S.~Martoiu$^{\rm 26a}$,
A.C.~Martyniuk$^{\rm 78}$,
M.~Marx$^{\rm 139}$,
F.~Marzano$^{\rm 133a}$,
A.~Marzin$^{\rm 30}$,
L.~Masetti$^{\rm 83}$,
T.~Mashimo$^{\rm 156}$,
R.~Mashinistov$^{\rm 96}$,
J.~Masik$^{\rm 84}$,
A.L.~Maslennikov$^{\rm 109}$$^{,c}$,
I.~Massa$^{\rm 20a,20b}$,
L.~Massa$^{\rm 20a,20b}$,
N.~Massol$^{\rm 5}$,
P.~Mastrandrea$^{\rm 149}$,
A.~Mastroberardino$^{\rm 37a,37b}$,
T.~Masubuchi$^{\rm 156}$,
P.~M\"attig$^{\rm 176}$,
J.~Mattmann$^{\rm 83}$,
J.~Maurer$^{\rm 26a}$,
S.J.~Maxfield$^{\rm 74}$,
D.A.~Maximov$^{\rm 109}$$^{,c}$,
R.~Mazini$^{\rm 152}$,
S.M.~Mazza$^{\rm 91a,91b}$,
L.~Mazzaferro$^{\rm 134a,134b}$,
G.~Mc~Goldrick$^{\rm 159}$,
S.P.~Mc~Kee$^{\rm 89}$,
A.~McCarn$^{\rm 89}$,
R.L.~McCarthy$^{\rm 149}$,
T.G.~McCarthy$^{\rm 29}$,
N.A.~McCubbin$^{\rm 131}$,
K.W.~McFarlane$^{\rm 56}$$^{,*}$,
J.A.~Mcfayden$^{\rm 78}$,
G.~Mchedlidze$^{\rm 54}$,
S.J.~McMahon$^{\rm 131}$,
R.A.~McPherson$^{\rm 170}$$^{,j}$,
M.~Medinnis$^{\rm 42}$,
S.~Meehan$^{\rm 146a}$,
S.~Mehlhase$^{\rm 100}$,
A.~Mehta$^{\rm 74}$,
K.~Meier$^{\rm 58a}$,
C.~Meineck$^{\rm 100}$,
B.~Meirose$^{\rm 41}$,
B.R.~Mellado~Garcia$^{\rm 146c}$,
F.~Meloni$^{\rm 17}$,
A.~Mengarelli$^{\rm 20a,20b}$,
S.~Menke$^{\rm 101}$,
E.~Meoni$^{\rm 162}$,
K.M.~Mercurio$^{\rm 57}$,
S.~Mergelmeyer$^{\rm 21}$,
P.~Mermod$^{\rm 49}$,
L.~Merola$^{\rm 104a,104b}$,
C.~Meroni$^{\rm 91a}$,
F.S.~Merritt$^{\rm 31}$,
A.~Messina$^{\rm 133a,133b}$,
J.~Metcalfe$^{\rm 25}$,
A.S.~Mete$^{\rm 164}$,
C.~Meyer$^{\rm 83}$,
C.~Meyer$^{\rm 122}$,
J-P.~Meyer$^{\rm 137}$,
J.~Meyer$^{\rm 107}$,
R.P.~Middleton$^{\rm 131}$,
S.~Miglioranzi$^{\rm 165a,165c}$,
L.~Mijovi\'{c}$^{\rm 21}$,
G.~Mikenberg$^{\rm 173}$,
M.~Mikestikova$^{\rm 127}$,
M.~Miku\v{z}$^{\rm 75}$,
M.~Milesi$^{\rm 88}$,
A.~Milic$^{\rm 30}$,
D.W.~Miller$^{\rm 31}$,
C.~Mills$^{\rm 46}$,
A.~Milov$^{\rm 173}$,
D.A.~Milstead$^{\rm 147a,147b}$,
A.A.~Minaenko$^{\rm 130}$,
Y.~Minami$^{\rm 156}$,
I.A.~Minashvili$^{\rm 65}$,
A.I.~Mincer$^{\rm 110}$,
B.~Mindur$^{\rm 38a}$,
M.~Mineev$^{\rm 65}$,
Y.~Ming$^{\rm 174}$,
L.M.~Mir$^{\rm 12}$,
T.~Mitani$^{\rm 172}$,
J.~Mitrevski$^{\rm 100}$,
V.A.~Mitsou$^{\rm 168}$,
A.~Miucci$^{\rm 49}$,
P.S.~Miyagawa$^{\rm 140}$,
J.U.~Mj\"ornmark$^{\rm 81}$,
T.~Moa$^{\rm 147a,147b}$,
K.~Mochizuki$^{\rm 85}$,
S.~Mohapatra$^{\rm 35}$,
W.~Mohr$^{\rm 48}$,
S.~Molander$^{\rm 147a,147b}$,
R.~Moles-Valls$^{\rm 168}$,
K.~M\"onig$^{\rm 42}$,
C.~Monini$^{\rm 55}$,
J.~Monk$^{\rm 36}$,
E.~Monnier$^{\rm 85}$,
J.~Montejo~Berlingen$^{\rm 12}$,
F.~Monticelli$^{\rm 71}$,
S.~Monzani$^{\rm 133a,133b}$,
R.W.~Moore$^{\rm 3}$,
N.~Morange$^{\rm 117}$,
D.~Moreno$^{\rm 163}$,
M.~Moreno~Ll\'acer$^{\rm 54}$,
P.~Morettini$^{\rm 50a}$,
M.~Morgenstern$^{\rm 44}$,
M.~Morii$^{\rm 57}$,
V.~Morisbak$^{\rm 119}$,
S.~Moritz$^{\rm 83}$,
A.K.~Morley$^{\rm 148}$,
G.~Mornacchi$^{\rm 30}$,
J.D.~Morris$^{\rm 76}$,
A.~Morton$^{\rm 53}$,
L.~Morvaj$^{\rm 103}$,
H.G.~Moser$^{\rm 101}$,
M.~Mosidze$^{\rm 51b}$,
J.~Moss$^{\rm 111}$,
K.~Motohashi$^{\rm 158}$,
R.~Mount$^{\rm 144}$,
E.~Mountricha$^{\rm 25}$,
S.V.~Mouraviev$^{\rm 96}$$^{,*}$,
E.J.W.~Moyse$^{\rm 86}$,
S.~Muanza$^{\rm 85}$,
R.D.~Mudd$^{\rm 18}$,
F.~Mueller$^{\rm 101}$,
J.~Mueller$^{\rm 125}$,
K.~Mueller$^{\rm 21}$,
R.S.P.~Mueller$^{\rm 100}$,
T.~Mueller$^{\rm 28}$,
D.~Muenstermann$^{\rm 49}$,
P.~Mullen$^{\rm 53}$,
Y.~Munwes$^{\rm 154}$,
J.A.~Murillo~Quijada$^{\rm 18}$,
W.J.~Murray$^{\rm 171,131}$,
H.~Musheghyan$^{\rm 54}$,
E.~Musto$^{\rm 153}$,
A.G.~Myagkov$^{\rm 130}$$^{,z}$,
M.~Myska$^{\rm 128}$,
O.~Nackenhorst$^{\rm 54}$,
J.~Nadal$^{\rm 54}$,
K.~Nagai$^{\rm 120}$,
R.~Nagai$^{\rm 158}$,
Y.~Nagai$^{\rm 85}$,
K.~Nagano$^{\rm 66}$,
A.~Nagarkar$^{\rm 111}$,
Y.~Nagasaka$^{\rm 59}$,
K.~Nagata$^{\rm 161}$,
M.~Nagel$^{\rm 101}$,
E.~Nagy$^{\rm 85}$,
A.M.~Nairz$^{\rm 30}$,
Y.~Nakahama$^{\rm 30}$,
K.~Nakamura$^{\rm 66}$,
T.~Nakamura$^{\rm 156}$,
I.~Nakano$^{\rm 112}$,
H.~Namasivayam$^{\rm 41}$,
G.~Nanava$^{\rm 21}$,
R.F.~Naranjo~Garcia$^{\rm 42}$,
R.~Narayan$^{\rm 58b}$,
T.~Naumann$^{\rm 42}$,
G.~Navarro$^{\rm 163}$,
R.~Nayyar$^{\rm 7}$,
H.A.~Neal$^{\rm 89}$,
P.Yu.~Nechaeva$^{\rm 96}$,
T.J.~Neep$^{\rm 84}$,
P.D.~Nef$^{\rm 144}$,
A.~Negri$^{\rm 121a,121b}$,
M.~Negrini$^{\rm 20a}$,
S.~Nektarijevic$^{\rm 106}$,
C.~Nellist$^{\rm 117}$,
A.~Nelson$^{\rm 164}$,
S.~Nemecek$^{\rm 127}$,
P.~Nemethy$^{\rm 110}$,
A.A.~Nepomuceno$^{\rm 24a}$,
M.~Nessi$^{\rm 30}$$^{,aa}$,
M.S.~Neubauer$^{\rm 166}$,
M.~Neumann$^{\rm 176}$,
R.M.~Neves$^{\rm 110}$,
P.~Nevski$^{\rm 25}$,
P.R.~Newman$^{\rm 18}$,
D.H.~Nguyen$^{\rm 6}$,
R.B.~Nickerson$^{\rm 120}$,
R.~Nicolaidou$^{\rm 137}$,
B.~Nicquevert$^{\rm 30}$,
J.~Nielsen$^{\rm 138}$,
N.~Nikiforou$^{\rm 35}$,
A.~Nikiforov$^{\rm 16}$,
V.~Nikolaenko$^{\rm 130}$$^{,z}$,
I.~Nikolic-Audit$^{\rm 80}$,
K.~Nikolopoulos$^{\rm 18}$,
J.K.~Nilsen$^{\rm 119}$,
P.~Nilsson$^{\rm 25}$,
Y.~Ninomiya$^{\rm 156}$,
A.~Nisati$^{\rm 133a}$,
R.~Nisius$^{\rm 101}$,
T.~Nobe$^{\rm 158}$,
M.~Nomachi$^{\rm 118}$,
I.~Nomidis$^{\rm 29}$,
T.~Nooney$^{\rm 76}$,
S.~Norberg$^{\rm 113}$,
M.~Nordberg$^{\rm 30}$,
O.~Novgorodova$^{\rm 44}$,
S.~Nowak$^{\rm 101}$,
M.~Nozaki$^{\rm 66}$,
L.~Nozka$^{\rm 115}$,
K.~Ntekas$^{\rm 10}$,
G.~Nunes~Hanninger$^{\rm 88}$,
T.~Nunnemann$^{\rm 100}$,
E.~Nurse$^{\rm 78}$,
F.~Nuti$^{\rm 88}$,
B.J.~O'Brien$^{\rm 46}$,
F.~O'grady$^{\rm 7}$,
D.C.~O'Neil$^{\rm 143}$,
V.~O'Shea$^{\rm 53}$,
F.G.~Oakham$^{\rm 29}$$^{,d}$,
H.~Oberlack$^{\rm 101}$,
T.~Obermann$^{\rm 21}$,
J.~Ocariz$^{\rm 80}$,
A.~Ochi$^{\rm 67}$,
I.~Ochoa$^{\rm 78}$,
S.~Oda$^{\rm 70}$,
S.~Odaka$^{\rm 66}$,
H.~Ogren$^{\rm 61}$,
A.~Oh$^{\rm 84}$,
S.H.~Oh$^{\rm 45}$,
C.C.~Ohm$^{\rm 15}$,
H.~Ohman$^{\rm 167}$,
H.~Oide$^{\rm 30}$,
W.~Okamura$^{\rm 118}$,
H.~Okawa$^{\rm 161}$,
Y.~Okumura$^{\rm 31}$,
T.~Okuyama$^{\rm 156}$,
A.~Olariu$^{\rm 26a}$,
S.A.~Olivares~Pino$^{\rm 46}$,
D.~Oliveira~Damazio$^{\rm 25}$,
E.~Oliver~Garcia$^{\rm 168}$,
A.~Olszewski$^{\rm 39}$,
J.~Olszowska$^{\rm 39}$,
A.~Onofre$^{\rm 126a,126e}$,
P.U.E.~Onyisi$^{\rm 31}$$^{,p}$,
C.J.~Oram$^{\rm 160a}$,
M.J.~Oreglia$^{\rm 31}$,
Y.~Oren$^{\rm 154}$,
D.~Orestano$^{\rm 135a,135b}$,
N.~Orlando$^{\rm 155}$,
C.~Oropeza~Barrera$^{\rm 53}$,
R.S.~Orr$^{\rm 159}$,
B.~Osculati$^{\rm 50a,50b}$,
R.~Ospanov$^{\rm 84}$,
G.~Otero~y~Garzon$^{\rm 27}$,
H.~Otono$^{\rm 70}$,
M.~Ouchrif$^{\rm 136d}$,
E.A.~Ouellette$^{\rm 170}$,
F.~Ould-Saada$^{\rm 119}$,
A.~Ouraou$^{\rm 137}$,
K.P.~Oussoren$^{\rm 107}$,
Q.~Ouyang$^{\rm 33a}$,
A.~Ovcharova$^{\rm 15}$,
M.~Owen$^{\rm 53}$,
R.E.~Owen$^{\rm 18}$,
V.E.~Ozcan$^{\rm 19a}$,
N.~Ozturk$^{\rm 8}$,
K.~Pachal$^{\rm 120}$,
A.~Pacheco~Pages$^{\rm 12}$,
C.~Padilla~Aranda$^{\rm 12}$,
M.~Pag\'{a}\v{c}ov\'{a}$^{\rm 48}$,
S.~Pagan~Griso$^{\rm 15}$,
E.~Paganis$^{\rm 140}$,
C.~Pahl$^{\rm 101}$,
F.~Paige$^{\rm 25}$,
P.~Pais$^{\rm 86}$,
K.~Pajchel$^{\rm 119}$,
G.~Palacino$^{\rm 160b}$,
S.~Palestini$^{\rm 30}$,
M.~Palka$^{\rm 38b}$,
D.~Pallin$^{\rm 34}$,
A.~Palma$^{\rm 126a,126b}$,
Y.B.~Pan$^{\rm 174}$,
E.~Panagiotopoulou$^{\rm 10}$,
C.E.~Pandini$^{\rm 80}$,
J.G.~Panduro~Vazquez$^{\rm 77}$,
P.~Pani$^{\rm 147a,147b}$,
S.~Panitkin$^{\rm 25}$,
L.~Paolozzi$^{\rm 134a,134b}$,
Th.D.~Papadopoulou$^{\rm 10}$,
K.~Papageorgiou$^{\rm 155}$,
A.~Paramonov$^{\rm 6}$,
D.~Paredes~Hernandez$^{\rm 155}$,
M.A.~Parker$^{\rm 28}$,
K.A.~Parker$^{\rm 140}$,
F.~Parodi$^{\rm 50a,50b}$,
J.A.~Parsons$^{\rm 35}$,
U.~Parzefall$^{\rm 48}$,
E.~Pasqualucci$^{\rm 133a}$,
S.~Passaggio$^{\rm 50a}$,
F.~Pastore$^{\rm 135a,135b}$$^{,*}$,
Fr.~Pastore$^{\rm 77}$,
G.~P\'asztor$^{\rm 29}$,
S.~Pataraia$^{\rm 176}$,
N.D.~Patel$^{\rm 151}$,
J.R.~Pater$^{\rm 84}$,
T.~Pauly$^{\rm 30}$,
J.~Pearce$^{\rm 170}$,
L.E.~Pedersen$^{\rm 36}$,
M.~Pedersen$^{\rm 119}$,
S.~Pedraza~Lopez$^{\rm 168}$,
R.~Pedro$^{\rm 126a,126b}$,
S.V.~Peleganchuk$^{\rm 109}$,
D.~Pelikan$^{\rm 167}$,
H.~Peng$^{\rm 33b}$,
B.~Penning$^{\rm 31}$,
J.~Penwell$^{\rm 61}$,
D.V.~Perepelitsa$^{\rm 25}$,
E.~Perez~Codina$^{\rm 160a}$,
M.T.~P\'erez~Garc\'ia-Esta\~n$^{\rm 168}$,
L.~Perini$^{\rm 91a,91b}$,
H.~Pernegger$^{\rm 30}$,
S.~Perrella$^{\rm 104a,104b}$,
R.~Peschke$^{\rm 42}$,
V.D.~Peshekhonov$^{\rm 65}$,
K.~Peters$^{\rm 30}$,
R.F.Y.~Peters$^{\rm 84}$,
B.A.~Petersen$^{\rm 30}$,
T.C.~Petersen$^{\rm 36}$,
E.~Petit$^{\rm 42}$,
A.~Petridis$^{\rm 147a,147b}$,
C.~Petridou$^{\rm 155}$,
E.~Petrolo$^{\rm 133a}$,
F.~Petrucci$^{\rm 135a,135b}$,
N.E.~Pettersson$^{\rm 158}$,
R.~Pezoa$^{\rm 32b}$,
P.W.~Phillips$^{\rm 131}$,
G.~Piacquadio$^{\rm 144}$,
E.~Pianori$^{\rm 171}$,
A.~Picazio$^{\rm 49}$,
E.~Piccaro$^{\rm 76}$,
M.~Piccinini$^{\rm 20a,20b}$,
M.A.~Pickering$^{\rm 120}$,
R.~Piegaia$^{\rm 27}$,
D.T.~Pignotti$^{\rm 111}$,
J.E.~Pilcher$^{\rm 31}$,
A.D.~Pilkington$^{\rm 78}$,
J.~Pina$^{\rm 126a,126b,126d}$,
M.~Pinamonti$^{\rm 165a,165c}$$^{,ab}$,
J.L.~Pinfold$^{\rm 3}$,
A.~Pingel$^{\rm 36}$,
B.~Pinto$^{\rm 126a}$,
S.~Pires$^{\rm 80}$,
M.~Pitt$^{\rm 173}$,
C.~Pizio$^{\rm 91a,91b}$,
L.~Plazak$^{\rm 145a}$,
M.-A.~Pleier$^{\rm 25}$,
V.~Pleskot$^{\rm 129}$,
E.~Plotnikova$^{\rm 65}$,
P.~Plucinski$^{\rm 147a,147b}$,
D.~Pluth$^{\rm 64}$,
R.~Poettgen$^{\rm 83}$,
L.~Poggioli$^{\rm 117}$,
D.~Pohl$^{\rm 21}$,
G.~Polesello$^{\rm 121a}$,
A.~Policicchio$^{\rm 37a,37b}$,
R.~Polifka$^{\rm 159}$,
A.~Polini$^{\rm 20a}$,
C.S.~Pollard$^{\rm 53}$,
V.~Polychronakos$^{\rm 25}$,
K.~Pomm\`es$^{\rm 30}$,
L.~Pontecorvo$^{\rm 133a}$,
B.G.~Pope$^{\rm 90}$,
G.A.~Popeneciu$^{\rm 26b}$,
D.S.~Popovic$^{\rm 13}$,
A.~Poppleton$^{\rm 30}$,
S.~Pospisil$^{\rm 128}$,
K.~Potamianos$^{\rm 15}$,
I.N.~Potrap$^{\rm 65}$,
C.J.~Potter$^{\rm 150}$,
C.T.~Potter$^{\rm 116}$,
G.~Poulard$^{\rm 30}$,
J.~Poveda$^{\rm 30}$,
V.~Pozdnyakov$^{\rm 65}$,
P.~Pralavorio$^{\rm 85}$,
A.~Pranko$^{\rm 15}$,
S.~Prasad$^{\rm 30}$,
S.~Prell$^{\rm 64}$,
D.~Price$^{\rm 84}$,
J.~Price$^{\rm 74}$,
L.E.~Price$^{\rm 6}$,
M.~Primavera$^{\rm 73a}$,
S.~Prince$^{\rm 87}$,
M.~Proissl$^{\rm 46}$,
K.~Prokofiev$^{\rm 60c}$,
F.~Prokoshin$^{\rm 32b}$,
E.~Protopapadaki$^{\rm 137}$,
S.~Protopopescu$^{\rm 25}$,
J.~Proudfoot$^{\rm 6}$,
M.~Przybycien$^{\rm 38a}$,
E.~Ptacek$^{\rm 116}$,
D.~Puddu$^{\rm 135a,135b}$,
E.~Pueschel$^{\rm 86}$,
D.~Puldon$^{\rm 149}$,
M.~Purohit$^{\rm 25}$$^{,ac}$,
P.~Puzo$^{\rm 117}$,
J.~Qian$^{\rm 89}$,
G.~Qin$^{\rm 53}$,
Y.~Qin$^{\rm 84}$,
A.~Quadt$^{\rm 54}$,
D.R.~Quarrie$^{\rm 15}$,
W.B.~Quayle$^{\rm 165a,165b}$,
M.~Queitsch-Maitland$^{\rm 84}$,
D.~Quilty$^{\rm 53}$,
A.~Qureshi$^{\rm 160b}$,
V.~Radeka$^{\rm 25}$,
V.~Radescu$^{\rm 42}$,
S.K.~Radhakrishnan$^{\rm 149}$,
P.~Radloff$^{\rm 116}$,
P.~Rados$^{\rm 88}$,
F.~Ragusa$^{\rm 91a,91b}$,
G.~Rahal$^{\rm 179}$,
S.~Rajagopalan$^{\rm 25}$,
M.~Rammensee$^{\rm 30}$,
C.~Rangel-Smith$^{\rm 167}$,
F.~Rauscher$^{\rm 100}$,
S.~Rave$^{\rm 83}$,
T.~Ravenscroft$^{\rm 53}$,
M.~Raymond$^{\rm 30}$,
A.L.~Read$^{\rm 119}$,
N.P.~Readioff$^{\rm 74}$,
D.M.~Rebuzzi$^{\rm 121a,121b}$,
A.~Redelbach$^{\rm 175}$,
G.~Redlinger$^{\rm 25}$,
R.~Reece$^{\rm 138}$,
K.~Reeves$^{\rm 41}$,
L.~Rehnisch$^{\rm 16}$,
H.~Reisin$^{\rm 27}$,
M.~Relich$^{\rm 164}$,
C.~Rembser$^{\rm 30}$,
H.~Ren$^{\rm 33a}$,
A.~Renaud$^{\rm 117}$,
M.~Rescigno$^{\rm 133a}$,
S.~Resconi$^{\rm 91a}$,
O.L.~Rezanova$^{\rm 109}$$^{,c}$,
P.~Reznicek$^{\rm 129}$,
R.~Rezvani$^{\rm 95}$,
R.~Richter$^{\rm 101}$,
E.~Richter-Was$^{\rm 38b}$,
O.~Ricken$^{\rm 21}$,
M.~Ridel$^{\rm 80}$,
P.~Rieck$^{\rm 16}$,
C.J.~Riegel$^{\rm 176}$,
J.~Rieger$^{\rm 54}$,
M.~Rijssenbeek$^{\rm 149}$,
A.~Rimoldi$^{\rm 121a,121b}$,
L.~Rinaldi$^{\rm 20a}$,
E.~Ritsch$^{\rm 62}$,
I.~Riu$^{\rm 12}$,
F.~Rizatdinova$^{\rm 114}$,
E.~Rizvi$^{\rm 76}$,
S.H.~Robertson$^{\rm 87}$$^{,j}$,
A.~Robichaud-Veronneau$^{\rm 87}$,
D.~Robinson$^{\rm 28}$,
J.E.M.~Robinson$^{\rm 84}$,
A.~Robson$^{\rm 53}$,
C.~Roda$^{\rm 124a,124b}$,
L.~Rodrigues$^{\rm 30}$,
S.~Roe$^{\rm 30}$,
O.~R{\o}hne$^{\rm 119}$,
S.~Rolli$^{\rm 162}$,
A.~Romaniouk$^{\rm 98}$,
M.~Romano$^{\rm 20a,20b}$,
S.M.~Romano~Saez$^{\rm 34}$,
E.~Romero~Adam$^{\rm 168}$,
N.~Rompotis$^{\rm 139}$,
M.~Ronzani$^{\rm 48}$,
L.~Roos$^{\rm 80}$,
E.~Ros$^{\rm 168}$,
S.~Rosati$^{\rm 133a}$,
K.~Rosbach$^{\rm 48}$,
P.~Rose$^{\rm 138}$,
P.L.~Rosendahl$^{\rm 14}$,
O.~Rosenthal$^{\rm 142}$,
V.~Rossetti$^{\rm 147a,147b}$,
E.~Rossi$^{\rm 104a,104b}$,
L.P.~Rossi$^{\rm 50a}$,
R.~Rosten$^{\rm 139}$,
M.~Rotaru$^{\rm 26a}$,
I.~Roth$^{\rm 173}$,
J.~Rothberg$^{\rm 139}$,
D.~Rousseau$^{\rm 117}$,
C.R.~Royon$^{\rm 137}$,
A.~Rozanov$^{\rm 85}$,
Y.~Rozen$^{\rm 153}$,
X.~Ruan$^{\rm 146c}$,
F.~Rubbo$^{\rm 144}$,
I.~Rubinskiy$^{\rm 42}$,
V.I.~Rud$^{\rm 99}$,
C.~Rudolph$^{\rm 44}$,
M.S.~Rudolph$^{\rm 159}$,
F.~R\"uhr$^{\rm 48}$,
A.~Ruiz-Martinez$^{\rm 30}$,
Z.~Rurikova$^{\rm 48}$,
N.A.~Rusakovich$^{\rm 65}$,
A.~Ruschke$^{\rm 100}$,
H.L.~Russell$^{\rm 139}$,
J.P.~Rutherfoord$^{\rm 7}$,
N.~Ruthmann$^{\rm 48}$,
Y.F.~Ryabov$^{\rm 123}$,
M.~Rybar$^{\rm 129}$,
G.~Rybkin$^{\rm 117}$,
N.C.~Ryder$^{\rm 120}$,
A.F.~Saavedra$^{\rm 151}$,
G.~Sabato$^{\rm 107}$,
S.~Sacerdoti$^{\rm 27}$,
A.~Saddique$^{\rm 3}$,
H.F-W.~Sadrozinski$^{\rm 138}$,
R.~Sadykov$^{\rm 65}$,
F.~Safai~Tehrani$^{\rm 133a}$,
M.~Saimpert$^{\rm 137}$,
H.~Sakamoto$^{\rm 156}$,
Y.~Sakurai$^{\rm 172}$,
G.~Salamanna$^{\rm 135a,135b}$,
A.~Salamon$^{\rm 134a}$,
M.~Saleem$^{\rm 113}$,
D.~Salek$^{\rm 107}$,
P.H.~Sales~De~Bruin$^{\rm 139}$,
D.~Salihagic$^{\rm 101}$,
A.~Salnikov$^{\rm 144}$,
J.~Salt$^{\rm 168}$,
D.~Salvatore$^{\rm 37a,37b}$,
F.~Salvatore$^{\rm 150}$,
A.~Salvucci$^{\rm 106}$,
A.~Salzburger$^{\rm 30}$,
D.~Sampsonidis$^{\rm 155}$,
A.~Sanchez$^{\rm 104a,104b}$,
J.~S\'anchez$^{\rm 168}$,
V.~Sanchez~Martinez$^{\rm 168}$,
H.~Sandaker$^{\rm 14}$,
R.L.~Sandbach$^{\rm 76}$,
H.G.~Sander$^{\rm 83}$,
M.P.~Sanders$^{\rm 100}$,
M.~Sandhoff$^{\rm 176}$,
C.~Sandoval$^{\rm 163}$,
R.~Sandstroem$^{\rm 101}$,
D.P.C.~Sankey$^{\rm 131}$,
A.~Sansoni$^{\rm 47}$,
C.~Santoni$^{\rm 34}$,
R.~Santonico$^{\rm 134a,134b}$,
H.~Santos$^{\rm 126a}$,
I.~Santoyo~Castillo$^{\rm 150}$,
K.~Sapp$^{\rm 125}$,
A.~Sapronov$^{\rm 65}$,
J.G.~Saraiva$^{\rm 126a,126d}$,
B.~Sarrazin$^{\rm 21}$,
O.~Sasaki$^{\rm 66}$,
Y.~Sasaki$^{\rm 156}$,
K.~Sato$^{\rm 161}$,
G.~Sauvage$^{\rm 5}$$^{,*}$,
E.~Sauvan$^{\rm 5}$,
G.~Savage$^{\rm 77}$,
P.~Savard$^{\rm 159}$$^{,d}$,
C.~Sawyer$^{\rm 120}$,
L.~Sawyer$^{\rm 79}$$^{,m}$,
J.~Saxon$^{\rm 31}$,
C.~Sbarra$^{\rm 20a}$,
A.~Sbrizzi$^{\rm 20a,20b}$,
T.~Scanlon$^{\rm 78}$,
D.A.~Scannicchio$^{\rm 164}$,
M.~Scarcella$^{\rm 151}$,
V.~Scarfone$^{\rm 37a,37b}$,
J.~Schaarschmidt$^{\rm 173}$,
P.~Schacht$^{\rm 101}$,
D.~Schaefer$^{\rm 30}$,
R.~Schaefer$^{\rm 42}$,
J.~Schaeffer$^{\rm 83}$,
S.~Schaepe$^{\rm 21}$,
S.~Schaetzel$^{\rm 58b}$,
U.~Sch\"afer$^{\rm 83}$,
A.C.~Schaffer$^{\rm 117}$,
D.~Schaile$^{\rm 100}$,
R.D.~Schamberger$^{\rm 149}$,
V.~Scharf$^{\rm 58a}$,
V.A.~Schegelsky$^{\rm 123}$,
D.~Scheirich$^{\rm 129}$,
M.~Schernau$^{\rm 164}$,
C.~Schiavi$^{\rm 50a,50b}$,
C.~Schillo$^{\rm 48}$,
M.~Schioppa$^{\rm 37a,37b}$,
S.~Schlenker$^{\rm 30}$,
E.~Schmidt$^{\rm 48}$,
K.~Schmieden$^{\rm 30}$,
C.~Schmitt$^{\rm 83}$,
S.~Schmitt$^{\rm 58b}$,
S.~Schmitt$^{\rm 42}$,
B.~Schneider$^{\rm 160a}$,
Y.J.~Schnellbach$^{\rm 74}$,
U.~Schnoor$^{\rm 44}$,
L.~Schoeffel$^{\rm 137}$,
A.~Schoening$^{\rm 58b}$,
B.D.~Schoenrock$^{\rm 90}$,
E.~Schopf$^{\rm 21}$,
A.L.S.~Schorlemmer$^{\rm 54}$,
M.~Schott$^{\rm 83}$,
D.~Schouten$^{\rm 160a}$,
J.~Schovancova$^{\rm 8}$,
S.~Schramm$^{\rm 159}$,
M.~Schreyer$^{\rm 175}$,
C.~Schroeder$^{\rm 83}$,
N.~Schuh$^{\rm 83}$,
M.J.~Schultens$^{\rm 21}$,
H.-C.~Schultz-Coulon$^{\rm 58a}$,
H.~Schulz$^{\rm 16}$,
M.~Schumacher$^{\rm 48}$,
B.A.~Schumm$^{\rm 138}$,
Ph.~Schune$^{\rm 137}$,
C.~Schwanenberger$^{\rm 84}$,
A.~Schwartzman$^{\rm 144}$,
T.A.~Schwarz$^{\rm 89}$,
Ph.~Schwegler$^{\rm 101}$,
Ph.~Schwemling$^{\rm 137}$,
R.~Schwienhorst$^{\rm 90}$,
J.~Schwindling$^{\rm 137}$,
T.~Schwindt$^{\rm 21}$,
M.~Schwoerer$^{\rm 5}$,
F.G.~Sciacca$^{\rm 17}$,
E.~Scifo$^{\rm 117}$,
G.~Sciolla$^{\rm 23}$,
F.~Scuri$^{\rm 124a,124b}$,
F.~Scutti$^{\rm 21}$,
J.~Searcy$^{\rm 89}$,
G.~Sedov$^{\rm 42}$,
E.~Sedykh$^{\rm 123}$,
P.~Seema$^{\rm 21}$,
S.C.~Seidel$^{\rm 105}$,
A.~Seiden$^{\rm 138}$,
F.~Seifert$^{\rm 128}$,
J.M.~Seixas$^{\rm 24a}$,
G.~Sekhniaidze$^{\rm 104a}$,
S.J.~Sekula$^{\rm 40}$,
K.E.~Selbach$^{\rm 46}$,
D.M.~Seliverstov$^{\rm 123}$$^{,*}$,
N.~Semprini-Cesari$^{\rm 20a,20b}$,
C.~Serfon$^{\rm 30}$,
L.~Serin$^{\rm 117}$,
L.~Serkin$^{\rm 54}$,
T.~Serre$^{\rm 85}$,
R.~Seuster$^{\rm 160a}$,
H.~Severini$^{\rm 113}$,
T.~Sfiligoj$^{\rm 75}$,
F.~Sforza$^{\rm 101}$,
A.~Sfyrla$^{\rm 30}$,
E.~Shabalina$^{\rm 54}$,
M.~Shamim$^{\rm 116}$,
L.Y.~Shan$^{\rm 33a}$,
R.~Shang$^{\rm 166}$,
J.T.~Shank$^{\rm 22}$,
M.~Shapiro$^{\rm 15}$,
P.B.~Shatalov$^{\rm 97}$,
K.~Shaw$^{\rm 165a,165b}$,
A.~Shcherbakova$^{\rm 147a,147b}$,
C.Y.~Shehu$^{\rm 150}$,
P.~Sherwood$^{\rm 78}$,
L.~Shi$^{\rm 152}$$^{,ad}$,
S.~Shimizu$^{\rm 67}$,
C.O.~Shimmin$^{\rm 164}$,
M.~Shimojima$^{\rm 102}$,
M.~Shiyakova$^{\rm 65}$,
A.~Shmeleva$^{\rm 96}$,
D.~Shoaleh~Saadi$^{\rm 95}$,
M.J.~Shochet$^{\rm 31}$,
S.~Shojaii$^{\rm 91a,91b}$,
S.~Shrestha$^{\rm 111}$,
E.~Shulga$^{\rm 98}$,
M.A.~Shupe$^{\rm 7}$,
S.~Shushkevich$^{\rm 42}$,
P.~Sicho$^{\rm 127}$,
O.~Sidiropoulou$^{\rm 175}$,
D.~Sidorov$^{\rm 114}$,
A.~Sidoti$^{\rm 20a,20b}$,
F.~Siegert$^{\rm 44}$,
Dj.~Sijacki$^{\rm 13}$,
J.~Silva$^{\rm 126a,126d}$,
Y.~Silver$^{\rm 154}$,
S.B.~Silverstein$^{\rm 147a}$,
V.~Simak$^{\rm 128}$,
O.~Simard$^{\rm 5}$,
Lj.~Simic$^{\rm 13}$,
S.~Simion$^{\rm 117}$,
E.~Simioni$^{\rm 83}$,
B.~Simmons$^{\rm 78}$,
D.~Simon$^{\rm 34}$,
R.~Simoniello$^{\rm 91a,91b}$,
P.~Sinervo$^{\rm 159}$,
N.B.~Sinev$^{\rm 116}$,
G.~Siragusa$^{\rm 175}$,
A.N.~Sisakyan$^{\rm 65}$$^{,*}$,
S.Yu.~Sivoklokov$^{\rm 99}$,
J.~Sj\"{o}lin$^{\rm 147a,147b}$,
T.B.~Sjursen$^{\rm 14}$,
M.B.~Skinner$^{\rm 72}$,
H.P.~Skottowe$^{\rm 57}$,
P.~Skubic$^{\rm 113}$,
M.~Slater$^{\rm 18}$,
T.~Slavicek$^{\rm 128}$,
M.~Slawinska$^{\rm 107}$,
K.~Sliwa$^{\rm 162}$,
V.~Smakhtin$^{\rm 173}$,
B.H.~Smart$^{\rm 46}$,
L.~Smestad$^{\rm 14}$,
S.Yu.~Smirnov$^{\rm 98}$,
Y.~Smirnov$^{\rm 98}$,
L.N.~Smirnova$^{\rm 99}$$^{,ae}$,
O.~Smirnova$^{\rm 81}$,
M.N.K.~Smith$^{\rm 35}$,
M.~Smizanska$^{\rm 72}$,
K.~Smolek$^{\rm 128}$,
A.A.~Snesarev$^{\rm 96}$,
G.~Snidero$^{\rm 76}$,
S.~Snyder$^{\rm 25}$,
R.~Sobie$^{\rm 170}$$^{,j}$,
F.~Socher$^{\rm 44}$,
A.~Soffer$^{\rm 154}$,
D.A.~Soh$^{\rm 152}$$^{,ad}$,
C.A.~Solans$^{\rm 30}$,
M.~Solar$^{\rm 128}$,
J.~Solc$^{\rm 128}$,
E.Yu.~Soldatov$^{\rm 98}$,
U.~Soldevila$^{\rm 168}$,
A.A.~Solodkov$^{\rm 130}$,
A.~Soloshenko$^{\rm 65}$,
O.V.~Solovyanov$^{\rm 130}$,
V.~Solovyev$^{\rm 123}$,
P.~Sommer$^{\rm 48}$,
H.Y.~Song$^{\rm 33b}$,
N.~Soni$^{\rm 1}$,
A.~Sood$^{\rm 15}$,
A.~Sopczak$^{\rm 128}$,
B.~Sopko$^{\rm 128}$,
V.~Sopko$^{\rm 128}$,
V.~Sorin$^{\rm 12}$,
D.~Sosa$^{\rm 58b}$,
M.~Sosebee$^{\rm 8}$,
C.L.~Sotiropoulou$^{\rm 155}$,
R.~Soualah$^{\rm 165a,165c}$,
P.~Soueid$^{\rm 95}$,
A.M.~Soukharev$^{\rm 109}$$^{,c}$,
D.~South$^{\rm 42}$,
S.~Spagnolo$^{\rm 73a,73b}$,
F.~Span\`o$^{\rm 77}$,
W.R.~Spearman$^{\rm 57}$,
F.~Spettel$^{\rm 101}$,
R.~Spighi$^{\rm 20a}$,
G.~Spigo$^{\rm 30}$,
L.A.~Spiller$^{\rm 88}$,
M.~Spousta$^{\rm 129}$,
T.~Spreitzer$^{\rm 159}$,
R.D.~St.~Denis$^{\rm 53}$$^{,*}$,
S.~Staerz$^{\rm 44}$,
J.~Stahlman$^{\rm 122}$,
R.~Stamen$^{\rm 58a}$,
S.~Stamm$^{\rm 16}$,
E.~Stanecka$^{\rm 39}$,
C.~Stanescu$^{\rm 135a}$,
M.~Stanescu-Bellu$^{\rm 42}$,
M.M.~Stanitzki$^{\rm 42}$,
S.~Stapnes$^{\rm 119}$,
E.A.~Starchenko$^{\rm 130}$,
J.~Stark$^{\rm 55}$,
P.~Staroba$^{\rm 127}$,
P.~Starovoitov$^{\rm 42}$,
R.~Staszewski$^{\rm 39}$,
P.~Stavina$^{\rm 145a}$$^{,*}$,
P.~Steinberg$^{\rm 25}$,
B.~Stelzer$^{\rm 143}$,
H.J.~Stelzer$^{\rm 30}$,
O.~Stelzer-Chilton$^{\rm 160a}$,
H.~Stenzel$^{\rm 52}$,
S.~Stern$^{\rm 101}$,
G.A.~Stewart$^{\rm 53}$,
J.A.~Stillings$^{\rm 21}$,
M.C.~Stockton$^{\rm 87}$,
M.~Stoebe$^{\rm 87}$,
G.~Stoicea$^{\rm 26a}$,
P.~Stolte$^{\rm 54}$,
S.~Stonjek$^{\rm 101}$,
A.R.~Stradling$^{\rm 8}$,
A.~Straessner$^{\rm 44}$,
M.E.~Stramaglia$^{\rm 17}$,
J.~Strandberg$^{\rm 148}$,
S.~Strandberg$^{\rm 147a,147b}$,
A.~Strandlie$^{\rm 119}$,
E.~Strauss$^{\rm 144}$,
M.~Strauss$^{\rm 113}$,
P.~Strizenec$^{\rm 145b}$,
R.~Str\"ohmer$^{\rm 175}$,
D.M.~Strom$^{\rm 116}$,
R.~Stroynowski$^{\rm 40}$,
A.~Strubig$^{\rm 106}$,
S.A.~Stucci$^{\rm 17}$,
B.~Stugu$^{\rm 14}$,
N.A.~Styles$^{\rm 42}$,
D.~Su$^{\rm 144}$,
J.~Su$^{\rm 125}$,
R.~Subramaniam$^{\rm 79}$,
A.~Succurro$^{\rm 12}$,
Y.~Sugaya$^{\rm 118}$,
C.~Suhr$^{\rm 108}$,
M.~Suk$^{\rm 128}$,
V.V.~Sulin$^{\rm 96}$,
S.~Sultansoy$^{\rm 4d}$,
T.~Sumida$^{\rm 68}$,
S.~Sun$^{\rm 57}$,
X.~Sun$^{\rm 33a}$,
J.E.~Sundermann$^{\rm 48}$,
K.~Suruliz$^{\rm 150}$,
G.~Susinno$^{\rm 37a,37b}$,
M.R.~Sutton$^{\rm 150}$,
S.~Suzuki$^{\rm 66}$,
Y.~Suzuki$^{\rm 66}$,
M.~Svatos$^{\rm 127}$,
S.~Swedish$^{\rm 169}$,
M.~Swiatlowski$^{\rm 144}$,
I.~Sykora$^{\rm 145a}$,
T.~Sykora$^{\rm 129}$,
D.~Ta$^{\rm 90}$,
C.~Taccini$^{\rm 135a,135b}$,
K.~Tackmann$^{\rm 42}$,
J.~Taenzer$^{\rm 159}$,
A.~Taffard$^{\rm 164}$,
R.~Tafirout$^{\rm 160a}$,
N.~Taiblum$^{\rm 154}$,
H.~Takai$^{\rm 25}$,
R.~Takashima$^{\rm 69}$,
H.~Takeda$^{\rm 67}$,
T.~Takeshita$^{\rm 141}$,
Y.~Takubo$^{\rm 66}$,
M.~Talby$^{\rm 85}$,
A.A.~Talyshev$^{\rm 109}$$^{,c}$,
J.Y.C.~Tam$^{\rm 175}$,
K.G.~Tan$^{\rm 88}$,
J.~Tanaka$^{\rm 156}$,
R.~Tanaka$^{\rm 117}$,
S.~Tanaka$^{\rm 132}$,
S.~Tanaka$^{\rm 66}$,
A.J.~Tanasijczuk$^{\rm 143}$,
B.B.~Tannenwald$^{\rm 111}$,
N.~Tannoury$^{\rm 21}$,
S.~Tapprogge$^{\rm 83}$,
S.~Tarem$^{\rm 153}$,
F.~Tarrade$^{\rm 29}$,
G.F.~Tartarelli$^{\rm 91a}$,
P.~Tas$^{\rm 129}$,
M.~Tasevsky$^{\rm 127}$,
T.~Tashiro$^{\rm 68}$,
E.~Tassi$^{\rm 37a,37b}$,
A.~Tavares~Delgado$^{\rm 126a,126b}$,
Y.~Tayalati$^{\rm 136d}$,
F.E.~Taylor$^{\rm 94}$,
G.N.~Taylor$^{\rm 88}$,
W.~Taylor$^{\rm 160b}$,
F.A.~Teischinger$^{\rm 30}$,
M.~Teixeira~Dias~Castanheira$^{\rm 76}$,
P.~Teixeira-Dias$^{\rm 77}$,
K.K.~Temming$^{\rm 48}$,
H.~Ten~Kate$^{\rm 30}$,
P.K.~Teng$^{\rm 152}$,
J.J.~Teoh$^{\rm 118}$,
F.~Tepel$^{\rm 176}$,
S.~Terada$^{\rm 66}$,
K.~Terashi$^{\rm 156}$,
J.~Terron$^{\rm 82}$,
S.~Terzo$^{\rm 101}$,
M.~Testa$^{\rm 47}$,
R.J.~Teuscher$^{\rm 159}$$^{,j}$,
J.~Therhaag$^{\rm 21}$,
T.~Theveneaux-Pelzer$^{\rm 34}$,
J.P.~Thomas$^{\rm 18}$,
J.~Thomas-Wilsker$^{\rm 77}$,
E.N.~Thompson$^{\rm 35}$,
P.D.~Thompson$^{\rm 18}$,
R.J.~Thompson$^{\rm 84}$,
A.S.~Thompson$^{\rm 53}$,
L.A.~Thomsen$^{\rm 36}$,
E.~Thomson$^{\rm 122}$,
M.~Thomson$^{\rm 28}$,
R.P.~Thun$^{\rm 89}$$^{,*}$,
M.J.~Tibbetts$^{\rm 15}$,
R.E.~Ticse~Torres$^{\rm 85}$,
V.O.~Tikhomirov$^{\rm 96}$$^{,af}$,
Yu.A.~Tikhonov$^{\rm 109}$$^{,c}$,
S.~Timoshenko$^{\rm 98}$,
E.~Tiouchichine$^{\rm 85}$,
P.~Tipton$^{\rm 177}$,
S.~Tisserant$^{\rm 85}$,
T.~Todorov$^{\rm 5}$$^{,*}$,
S.~Todorova-Nova$^{\rm 129}$,
J.~Tojo$^{\rm 70}$,
S.~Tok\'ar$^{\rm 145a}$,
K.~Tokushuku$^{\rm 66}$,
K.~Tollefson$^{\rm 90}$,
E.~Tolley$^{\rm 57}$,
L.~Tomlinson$^{\rm 84}$,
M.~Tomoto$^{\rm 103}$,
L.~Tompkins$^{\rm 144}$$^{,ag}$,
K.~Toms$^{\rm 105}$,
E.~Torrence$^{\rm 116}$,
H.~Torres$^{\rm 143}$,
E.~Torr\'o~Pastor$^{\rm 168}$,
J.~Toth$^{\rm 85}$$^{,ah}$,
F.~Touchard$^{\rm 85}$,
D.R.~Tovey$^{\rm 140}$,
T.~Trefzger$^{\rm 175}$,
L.~Tremblet$^{\rm 30}$,
A.~Tricoli$^{\rm 30}$,
I.M.~Trigger$^{\rm 160a}$,
S.~Trincaz-Duvoid$^{\rm 80}$,
M.F.~Tripiana$^{\rm 12}$,
W.~Trischuk$^{\rm 159}$,
B.~Trocm\'e$^{\rm 55}$,
C.~Troncon$^{\rm 91a}$,
M.~Trottier-McDonald$^{\rm 15}$,
M.~Trovatelli$^{\rm 135a,135b}$,
P.~True$^{\rm 90}$,
M.~Trzebinski$^{\rm 39}$,
A.~Trzupek$^{\rm 39}$,
C.~Tsarouchas$^{\rm 30}$,
J.C-L.~Tseng$^{\rm 120}$,
P.V.~Tsiareshka$^{\rm 92}$,
D.~Tsionou$^{\rm 155}$,
G.~Tsipolitis$^{\rm 10}$,
N.~Tsirintanis$^{\rm 9}$,
S.~Tsiskaridze$^{\rm 12}$,
V.~Tsiskaridze$^{\rm 48}$,
E.G.~Tskhadadze$^{\rm 51a}$,
I.I.~Tsukerman$^{\rm 97}$,
V.~Tsulaia$^{\rm 15}$,
S.~Tsuno$^{\rm 66}$,
D.~Tsybychev$^{\rm 149}$,
A.~Tudorache$^{\rm 26a}$,
V.~Tudorache$^{\rm 26a}$,
A.N.~Tuna$^{\rm 122}$,
S.A.~Tupputi$^{\rm 20a,20b}$,
S.~Turchikhin$^{\rm 99}$$^{,ae}$,
D.~Turecek$^{\rm 128}$,
I.~Turk~Cakir$^{\rm 4c}$,
R.~Turra$^{\rm 91a,91b}$,
A.J.~Turvey$^{\rm 40}$,
P.M.~Tuts$^{\rm 35}$,
A.~Tykhonov$^{\rm 49}$,
M.~Tylmad$^{\rm 147a,147b}$,
M.~Tyndel$^{\rm 131}$,
I.~Ueda$^{\rm 156}$,
R.~Ueno$^{\rm 29}$,
M.~Ughetto$^{\rm 147a,147b}$,
M.~Ugland$^{\rm 14}$,
M.~Uhlenbrock$^{\rm 21}$,
F.~Ukegawa$^{\rm 161}$,
G.~Unal$^{\rm 30}$,
A.~Undrus$^{\rm 25}$,
G.~Unel$^{\rm 164}$,
F.C.~Ungaro$^{\rm 48}$,
Y.~Unno$^{\rm 66}$,
C.~Unverdorben$^{\rm 100}$,
J.~Urban$^{\rm 145b}$,
P.~Urquijo$^{\rm 88}$,
P.~Urrejola$^{\rm 83}$,
G.~Usai$^{\rm 8}$,
A.~Usanova$^{\rm 62}$,
L.~Vacavant$^{\rm 85}$,
V.~Vacek$^{\rm 128}$,
B.~Vachon$^{\rm 87}$,
N.~Valencic$^{\rm 107}$,
S.~Valentinetti$^{\rm 20a,20b}$,
A.~Valero$^{\rm 168}$,
L.~Valery$^{\rm 12}$,
S.~Valkar$^{\rm 129}$,
E.~Valladolid~Gallego$^{\rm 168}$,
S.~Vallecorsa$^{\rm 49}$,
J.A.~Valls~Ferrer$^{\rm 168}$,
W.~Van~Den~Wollenberg$^{\rm 107}$,
P.C.~Van~Der~Deijl$^{\rm 107}$,
R.~van~der~Geer$^{\rm 107}$,
H.~van~der~Graaf$^{\rm 107}$,
R.~Van~Der~Leeuw$^{\rm 107}$,
N.~van~Eldik$^{\rm 153}$,
P.~van~Gemmeren$^{\rm 6}$,
J.~Van~Nieuwkoop$^{\rm 143}$,
I.~van~Vulpen$^{\rm 107}$,
M.C.~van~Woerden$^{\rm 30}$,
M.~Vanadia$^{\rm 133a,133b}$,
W.~Vandelli$^{\rm 30}$,
R.~Vanguri$^{\rm 122}$,
A.~Vaniachine$^{\rm 6}$,
F.~Vannucci$^{\rm 80}$,
G.~Vardanyan$^{\rm 178}$,
R.~Vari$^{\rm 133a}$,
E.W.~Varnes$^{\rm 7}$,
T.~Varol$^{\rm 40}$,
D.~Varouchas$^{\rm 80}$,
A.~Vartapetian$^{\rm 8}$,
K.E.~Varvell$^{\rm 151}$,
F.~Vazeille$^{\rm 34}$,
T.~Vazquez~Schroeder$^{\rm 54}$,
J.~Veatch$^{\rm 7}$,
F.~Veloso$^{\rm 126a,126c}$,
T.~Velz$^{\rm 21}$,
S.~Veneziano$^{\rm 133a}$,
A.~Ventura$^{\rm 73a,73b}$,
D.~Ventura$^{\rm 86}$,
M.~Venturi$^{\rm 170}$,
N.~Venturi$^{\rm 159}$,
A.~Venturini$^{\rm 23}$,
V.~Vercesi$^{\rm 121a}$,
M.~Verducci$^{\rm 133a,133b}$,
W.~Verkerke$^{\rm 107}$,
J.C.~Vermeulen$^{\rm 107}$,
A.~Vest$^{\rm 44}$,
M.C.~Vetterli$^{\rm 143}$$^{,d}$,
O.~Viazlo$^{\rm 81}$,
I.~Vichou$^{\rm 166}$,
T.~Vickey$^{\rm 140}$,
O.E.~Vickey~Boeriu$^{\rm 140}$,
G.H.A.~Viehhauser$^{\rm 120}$,
S.~Viel$^{\rm 15}$,
R.~Vigne$^{\rm 30}$,
M.~Villa$^{\rm 20a,20b}$,
M.~Villaplana~Perez$^{\rm 91a,91b}$,
E.~Vilucchi$^{\rm 47}$,
M.G.~Vincter$^{\rm 29}$,
V.B.~Vinogradov$^{\rm 65}$,
I.~Vivarelli$^{\rm 150}$,
F.~Vives~Vaque$^{\rm 3}$,
S.~Vlachos$^{\rm 10}$,
D.~Vladoiu$^{\rm 100}$,
M.~Vlasak$^{\rm 128}$,
M.~Vogel$^{\rm 32a}$,
P.~Vokac$^{\rm 128}$,
G.~Volpi$^{\rm 124a,124b}$,
M.~Volpi$^{\rm 88}$,
H.~von~der~Schmitt$^{\rm 101}$,
H.~von~Radziewski$^{\rm 48}$,
E.~von~Toerne$^{\rm 21}$,
V.~Vorobel$^{\rm 129}$,
K.~Vorobev$^{\rm 98}$,
M.~Vos$^{\rm 168}$,
R.~Voss$^{\rm 30}$,
J.H.~Vossebeld$^{\rm 74}$,
N.~Vranjes$^{\rm 13}$,
M.~Vranjes~Milosavljevic$^{\rm 13}$,
V.~Vrba$^{\rm 127}$,
M.~Vreeswijk$^{\rm 107}$,
R.~Vuillermet$^{\rm 30}$,
I.~Vukotic$^{\rm 31}$,
Z.~Vykydal$^{\rm 128}$,
P.~Wagner$^{\rm 21}$,
W.~Wagner$^{\rm 176}$,
H.~Wahlberg$^{\rm 71}$,
S.~Wahrmund$^{\rm 44}$,
J.~Wakabayashi$^{\rm 103}$,
J.~Walder$^{\rm 72}$,
R.~Walker$^{\rm 100}$,
W.~Walkowiak$^{\rm 142}$,
C.~Wang$^{\rm 33c}$,
F.~Wang$^{\rm 174}$,
H.~Wang$^{\rm 15}$,
H.~Wang$^{\rm 40}$,
J.~Wang$^{\rm 42}$,
J.~Wang$^{\rm 33a}$,
K.~Wang$^{\rm 87}$,
R.~Wang$^{\rm 6}$,
S.M.~Wang$^{\rm 152}$,
T.~Wang$^{\rm 21}$,
X.~Wang$^{\rm 177}$,
C.~Wanotayaroj$^{\rm 116}$,
A.~Warburton$^{\rm 87}$,
C.P.~Ward$^{\rm 28}$,
D.R.~Wardrope$^{\rm 78}$,
M.~Warsinsky$^{\rm 48}$,
A.~Washbrook$^{\rm 46}$,
C.~Wasicki$^{\rm 42}$,
P.M.~Watkins$^{\rm 18}$,
A.T.~Watson$^{\rm 18}$,
I.J.~Watson$^{\rm 151}$,
M.F.~Watson$^{\rm 18}$,
G.~Watts$^{\rm 139}$,
S.~Watts$^{\rm 84}$,
B.M.~Waugh$^{\rm 78}$,
S.~Webb$^{\rm 84}$,
M.S.~Weber$^{\rm 17}$,
S.W.~Weber$^{\rm 175}$,
J.S.~Webster$^{\rm 31}$,
A.R.~Weidberg$^{\rm 120}$,
B.~Weinert$^{\rm 61}$,
J.~Weingarten$^{\rm 54}$,
C.~Weiser$^{\rm 48}$,
H.~Weits$^{\rm 107}$,
P.S.~Wells$^{\rm 30}$,
T.~Wenaus$^{\rm 25}$,
T.~Wengler$^{\rm 30}$,
S.~Wenig$^{\rm 30}$,
N.~Wermes$^{\rm 21}$,
M.~Werner$^{\rm 48}$,
P.~Werner$^{\rm 30}$,
M.~Wessels$^{\rm 58a}$,
J.~Wetter$^{\rm 162}$,
K.~Whalen$^{\rm 29}$,
A.M.~Wharton$^{\rm 72}$,
A.~White$^{\rm 8}$,
M.J.~White$^{\rm 1}$,
R.~White$^{\rm 32b}$,
S.~White$^{\rm 124a,124b}$,
D.~Whiteson$^{\rm 164}$,
F.J.~Wickens$^{\rm 131}$,
W.~Wiedenmann$^{\rm 174}$,
M.~Wielers$^{\rm 131}$,
P.~Wienemann$^{\rm 21}$,
C.~Wiglesworth$^{\rm 36}$,
L.A.M.~Wiik-Fuchs$^{\rm 21}$,
A.~Wildauer$^{\rm 101}$,
H.G.~Wilkens$^{\rm 30}$,
H.H.~Williams$^{\rm 122}$,
S.~Williams$^{\rm 107}$,
C.~Willis$^{\rm 90}$,
S.~Willocq$^{\rm 86}$,
A.~Wilson$^{\rm 89}$,
J.A.~Wilson$^{\rm 18}$,
I.~Wingerter-Seez$^{\rm 5}$,
F.~Winklmeier$^{\rm 116}$,
B.T.~Winter$^{\rm 21}$,
M.~Wittgen$^{\rm 144}$,
J.~Wittkowski$^{\rm 100}$,
S.J.~Wollstadt$^{\rm 83}$,
M.W.~Wolter$^{\rm 39}$,
H.~Wolters$^{\rm 126a,126c}$,
B.K.~Wosiek$^{\rm 39}$,
J.~Wotschack$^{\rm 30}$,
M.J.~Woudstra$^{\rm 84}$,
K.W.~Wozniak$^{\rm 39}$,
M.~Wu$^{\rm 55}$,
M.~Wu$^{\rm 31}$,
S.L.~Wu$^{\rm 174}$,
X.~Wu$^{\rm 49}$,
Y.~Wu$^{\rm 89}$,
T.R.~Wyatt$^{\rm 84}$,
B.M.~Wynne$^{\rm 46}$,
S.~Xella$^{\rm 36}$,
D.~Xu$^{\rm 33a}$,
L.~Xu$^{\rm 33b}$$^{,ai}$,
B.~Yabsley$^{\rm 151}$,
S.~Yacoob$^{\rm 146b}$$^{,aj}$,
R.~Yakabe$^{\rm 67}$,
M.~Yamada$^{\rm 66}$,
Y.~Yamaguchi$^{\rm 118}$,
A.~Yamamoto$^{\rm 66}$,
S.~Yamamoto$^{\rm 156}$,
T.~Yamanaka$^{\rm 156}$,
K.~Yamauchi$^{\rm 103}$,
Y.~Yamazaki$^{\rm 67}$,
Z.~Yan$^{\rm 22}$,
H.~Yang$^{\rm 33e}$,
H.~Yang$^{\rm 174}$,
Y.~Yang$^{\rm 152}$,
L.~Yao$^{\rm 33a}$,
W-M.~Yao$^{\rm 15}$,
Y.~Yasu$^{\rm 66}$,
E.~Yatsenko$^{\rm 42}$,
K.H.~Yau~Wong$^{\rm 21}$,
J.~Ye$^{\rm 40}$,
S.~Ye$^{\rm 25}$,
I.~Yeletskikh$^{\rm 65}$,
A.L.~Yen$^{\rm 57}$,
E.~Yildirim$^{\rm 42}$,
K.~Yorita$^{\rm 172}$,
R.~Yoshida$^{\rm 6}$,
K.~Yoshihara$^{\rm 122}$,
C.~Young$^{\rm 144}$,
C.J.S.~Young$^{\rm 30}$,
S.~Youssef$^{\rm 22}$,
D.R.~Yu$^{\rm 15}$,
J.~Yu$^{\rm 8}$,
J.M.~Yu$^{\rm 89}$,
J.~Yu$^{\rm 114}$,
L.~Yuan$^{\rm 67}$,
A.~Yurkewicz$^{\rm 108}$,
I.~Yusuff$^{\rm 28}$$^{,ak}$,
B.~Zabinski$^{\rm 39}$,
R.~Zaidan$^{\rm 63}$,
A.M.~Zaitsev$^{\rm 130}$$^{,z}$,
A.~Zaman$^{\rm 149}$,
S.~Zambito$^{\rm 23}$,
L.~Zanello$^{\rm 133a,133b}$,
D.~Zanzi$^{\rm 88}$,
C.~Zeitnitz$^{\rm 176}$,
M.~Zeman$^{\rm 128}$,
A.~Zemla$^{\rm 38a}$,
K.~Zengel$^{\rm 23}$,
O.~Zenin$^{\rm 130}$,
T.~\v{Z}eni\v{s}$^{\rm 145a}$,
D.~Zerwas$^{\rm 117}$,
D.~Zhang$^{\rm 89}$,
F.~Zhang$^{\rm 174}$,
J.~Zhang$^{\rm 6}$,
L.~Zhang$^{\rm 152}$,
R.~Zhang$^{\rm 33b}$,
X.~Zhang$^{\rm 33d}$,
Z.~Zhang$^{\rm 117}$,
X.~Zhao$^{\rm 40}$,
Y.~Zhao$^{\rm 33d,117}$,
Z.~Zhao$^{\rm 33b}$,
A.~Zhemchugov$^{\rm 65}$,
J.~Zhong$^{\rm 120}$,
B.~Zhou$^{\rm 89}$,
C.~Zhou$^{\rm 45}$,
L.~Zhou$^{\rm 35}$,
L.~Zhou$^{\rm 40}$,
N.~Zhou$^{\rm 164}$,
C.G.~Zhu$^{\rm 33d}$,
H.~Zhu$^{\rm 33a}$,
J.~Zhu$^{\rm 89}$,
Y.~Zhu$^{\rm 33b}$,
X.~Zhuang$^{\rm 33a}$,
K.~Zhukov$^{\rm 96}$,
A.~Zibell$^{\rm 175}$,
D.~Zieminska$^{\rm 61}$,
N.I.~Zimine$^{\rm 65}$,
C.~Zimmermann$^{\rm 83}$,
R.~Zimmermann$^{\rm 21}$,
S.~Zimmermann$^{\rm 48}$,
Z.~Zinonos$^{\rm 54}$,
M.~Zinser$^{\rm 83}$,
M.~Ziolkowski$^{\rm 142}$,
L.~\v{Z}ivkovi\'{c}$^{\rm 13}$,
G.~Zobernig$^{\rm 174}$,
A.~Zoccoli$^{\rm 20a,20b}$,
M.~zur~Nedden$^{\rm 16}$,
G.~Zurzolo$^{\rm 104a,104b}$,
L.~Zwalinski$^{\rm 30}$.
\bigskip
\\
$^{1}$ Department of Physics, University of Adelaide, Adelaide, Australia\\
$^{2}$ Physics Department, SUNY Albany, Albany NY, United States of America\\
$^{3}$ Department of Physics, University of Alberta, Edmonton AB, Canada\\
$^{4}$ $^{(a)}$ Department of Physics, Ankara University, Ankara; $^{(c)}$ Istanbul Aydin University, Istanbul; $^{(d)}$ Division of Physics, TOBB University of Economics and Technology, Ankara, Turkey\\
$^{5}$ LAPP, CNRS/IN2P3 and Universit{\'e} de Savoie, Annecy-le-Vieux, France\\
$^{6}$ High Energy Physics Division, Argonne National Laboratory, Argonne IL, United States of America\\
$^{7}$ Department of Physics, University of Arizona, Tucson AZ, United States of America\\
$^{8}$ Department of Physics, The University of Texas at Arlington, Arlington TX, United States of America\\
$^{9}$ Physics Department, University of Athens, Athens, Greece\\
$^{10}$ Physics Department, National Technical University of Athens, Zografou, Greece\\
$^{11}$ Institute of Physics, Azerbaijan Academy of Sciences, Baku, Azerbaijan\\
$^{12}$ Institut de F{\'\i}sica d'Altes Energies and Departament de F{\'\i}sica de la Universitat Aut{\`o}noma de Barcelona, Barcelona, Spain\\
$^{13}$ Institute of Physics, University of Belgrade, Belgrade, Serbia\\
$^{14}$ Department for Physics and Technology, University of Bergen, Bergen, Norway\\
$^{15}$ Physics Division, Lawrence Berkeley National Laboratory and University of California, Berkeley CA, United States of America\\
$^{16}$ Department of Physics, Humboldt University, Berlin, Germany\\
$^{17}$ Albert Einstein Center for Fundamental Physics and Laboratory for High Energy Physics, University of Bern, Bern, Switzerland\\
$^{18}$ School of Physics and Astronomy, University of Birmingham, Birmingham, United Kingdom\\
$^{19}$ $^{(a)}$ Department of Physics, Bogazici University, Istanbul; $^{(b)}$ Department of Physics, Dogus University, Istanbul; $^{(c)}$ Department of Physics Engineering, Gaziantep University, Gaziantep, Turkey\\
$^{20}$ $^{(a)}$ INFN Sezione di Bologna; $^{(b)}$ Dipartimento di Fisica e Astronomia, Universit{\`a} di Bologna, Bologna, Italy\\
$^{21}$ Physikalisches Institut, University of Bonn, Bonn, Germany\\
$^{22}$ Department of Physics, Boston University, Boston MA, United States of America\\
$^{23}$ Department of Physics, Brandeis University, Waltham MA, United States of America\\
$^{24}$ $^{(a)}$ Universidade Federal do Rio De Janeiro COPPE/EE/IF, Rio de Janeiro; $^{(b)}$ Electrical Circuits Department, Federal University of Juiz de Fora (UFJF), Juiz de Fora; $^{(c)}$ Federal University of Sao Joao del Rei (UFSJ), Sao Joao del Rei; $^{(d)}$ Instituto de Fisica, Universidade de Sao Paulo, Sao Paulo, Brazil\\
$^{25}$ Physics Department, Brookhaven National Laboratory, Upton NY, United States of America\\
$^{26}$ $^{(a)}$ National Institute of Physics and Nuclear Engineering, Bucharest; $^{(b)}$ National Institute for Research and Development of Isotopic and Molecular Technologies, Physics Department, Cluj Napoca; $^{(c)}$ University Politehnica Bucharest, Bucharest; $^{(d)}$ West University in Timisoara, Timisoara, Romania\\
$^{27}$ Departamento de F{\'\i}sica, Universidad de Buenos Aires, Buenos Aires, Argentina\\
$^{28}$ Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{29}$ Department of Physics, Carleton University, Ottawa ON, Canada\\
$^{30}$ CERN, Geneva, Switzerland\\
$^{31}$ Enrico Fermi Institute, University of Chicago, Chicago IL, United States of America\\
$^{32}$ $^{(a)}$ Departamento de F{\'\i}sica, Pontificia Universidad Cat{\'o}lica de Chile, Santiago; $^{(b)}$ Departamento de F{\'\i}sica, Universidad T{\'e}cnica Federico Santa Mar{\'\i}a, Valpara{\'\i}so, Chile\\
$^{33}$ $^{(a)}$ Institute of High Energy Physics, Chinese Academy of Sciences, Beijing; $^{(b)}$ Department of Modern Physics, University of Science and Technology of China, Anhui; $^{(c)}$ Department of Physics, Nanjing University, Jiangsu; $^{(d)}$ School of Physics, Shandong University, Shandong; $^{(e)}$ Department of Physics and Astronomy, Shanghai Key Laboratory for  Particle Physics and Cosmology, Shanghai Jiao Tong University, Shanghai; $^{(f)}$ Physics Department, Tsinghua University, Beijing 100084, China\\
$^{34}$ Laboratoire de Physique Corpusculaire, Clermont Universit{\'e} and Universit{\'e} Blaise Pascal and CNRS/IN2P3, Clermont-Ferrand, France\\
$^{35}$ Nevis Laboratory, Columbia University, Irvington NY, United States of America\\
$^{36}$ Niels Bohr Institute, University of Copenhagen, Kobenhavn, Denmark\\
$^{37}$ $^{(a)}$ INFN Gruppo Collegato di Cosenza, Laboratori Nazionali di Frascati; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} della Calabria, Rende, Italy\\
$^{38}$ $^{(a)}$ AGH University of Science and Technology, Faculty of Physics and Applied Computer Science, Krakow; $^{(b)}$ Marian Smoluchowski Institute of Physics, Jagiellonian University, Krakow, Poland\\
$^{39}$ Institute of Nuclear Physics Polish Academy of Sciences, Krakow, Poland\\
$^{40}$ Physics Department, Southern Methodist University, Dallas TX, United States of America\\
$^{41}$ Physics Department, University of Texas at Dallas, Richardson TX, United States of America\\
$^{42}$ DESY, Hamburg and Zeuthen, Germany\\
$^{43}$ Institut f{\"u}r Experimentelle Physik IV, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{44}$ Institut f{\"u}r Kern-{~}und Teilchenphysik, Technische Universit{\"a}t Dresden, Dresden, Germany\\
$^{45}$ Department of Physics, Duke University, Durham NC, United States of America\\
$^{46}$ SUPA - School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{47}$ INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{48}$ Fakult{\"a}t f{\"u}r Mathematik und Physik, Albert-Ludwigs-Universit{\"a}t, Freiburg, Germany\\
$^{49}$ Section de Physique, Universit{\'e} de Gen{\`e}ve, Geneva, Switzerland\\
$^{50}$ $^{(a)}$ INFN Sezione di Genova; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Genova, Genova, Italy\\
$^{51}$ $^{(a)}$ E. Andronikashvili Institute of Physics, Iv. Javakhishvili Tbilisi State University, Tbilisi; $^{(b)}$ High Energy Physics Institute, Tbilisi State University, Tbilisi, Georgia\\
$^{52}$ II Physikalisches Institut, Justus-Liebig-Universit{\"a}t Giessen, Giessen, Germany\\
$^{53}$ SUPA - School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{54}$ II Physikalisches Institut, Georg-August-Universit{\"a}t, G{\"o}ttingen, Germany\\
$^{55}$ Laboratoire de Physique Subatomique et de Cosmologie, Universit{\'e} Grenoble-Alpes, CNRS/IN2P3, Grenoble, France\\
$^{56}$ Department of Physics, Hampton University, Hampton VA, United States of America\\
$^{57}$ Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge MA, United States of America\\
$^{58}$ $^{(a)}$ Kirchhoff-Institut f{\"u}r Physik, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg; $^{(b)}$ Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg; $^{(c)}$ ZITI Institut f{\"u}r technische Informatik, Ruprecht-Karls-Universit{\"a}t Heidelberg, Mannheim, Germany\\
$^{59}$ Faculty of Applied Information Science, Hiroshima Institute of Technology, Hiroshima, Japan\\
$^{60}$ $^{(a)}$ Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong; $^{(b)}$ Department of Physics, The University of Hong Kong, Hong Kong; $^{(c)}$ Department of Physics, The Hong Kong University of Science and Technology, Clear Water Bay, Kowloon, Hong Kong, China\\
$^{61}$ Department of Physics, Indiana University, Bloomington IN, United States of America\\
$^{62}$ Institut f{\"u}r Astro-{~}und Teilchenphysik, Leopold-Franzens-Universit{\"a}t, Innsbruck, Austria\\
$^{63}$ University of Iowa, Iowa City IA, United States of America\\
$^{64}$ Department of Physics and Astronomy, Iowa State University, Ames IA, United States of America\\
$^{65}$ Joint Institute for Nuclear Research, JINR Dubna, Dubna, Russia\\
$^{66}$ KEK, High Energy Accelerator Research Organization, Tsukuba, Japan\\
$^{67}$ Graduate School of Science, Kobe University, Kobe, Japan\\
$^{68}$ Faculty of Science, Kyoto University, Kyoto, Japan\\
$^{69}$ Kyoto University of Education, Kyoto, Japan\\
$^{70}$ Department of Physics, Kyushu University, Fukuoka, Japan\\
$^{71}$ Instituto de F{\'\i}sica La Plata, Universidad Nacional de La Plata and CONICET, La Plata, Argentina\\
$^{72}$ Physics Department, Lancaster University, Lancaster, United Kingdom\\
$^{73}$ $^{(a)}$ INFN Sezione di Lecce; $^{(b)}$ Dipartimento di Matematica e Fisica, Universit{\`a} del Salento, Lecce, Italy\\
$^{74}$ Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{75}$ Department of Physics, Jo{\v{z}}ef Stefan Institute and University of Ljubljana, Ljubljana, Slovenia\\
$^{76}$ School of Physics and Astronomy, Queen Mary University of London, London, United Kingdom\\
$^{77}$ Department of Physics, Royal Holloway University of London, Surrey, United Kingdom\\
$^{78}$ Department of Physics and Astronomy, University College London, London, United Kingdom\\
$^{79}$ Louisiana Tech University, Ruston LA, United States of America\\
$^{80}$ Laboratoire de Physique Nucl{\'e}aire et de Hautes Energies, UPMC and Universit{\'e} Paris-Diderot and CNRS/IN2P3, Paris, France\\
$^{81}$ Fysiska institutionen, Lunds universitet, Lund, Sweden\\
$^{82}$ Departamento de Fisica Teorica C-15, Universidad Autonoma de Madrid, Madrid, Spain\\
$^{83}$ Institut f{\"u}r Physik, Universit{\"a}t Mainz, Mainz, Germany\\
$^{84}$ School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{85}$ CPPM, Aix-Marseille Universit{\'e} and CNRS/IN2P3, Marseille, France\\
$^{86}$ Department of Physics, University of Massachusetts, Amherst MA, United States of America\\
$^{87}$ Department of Physics, McGill University, Montreal QC, Canada\\
$^{88}$ School of Physics, University of Melbourne, Victoria, Australia\\
$^{89}$ Department of Physics, The University of Michigan, Ann Arbor MI, United States of America\\
$^{90}$ Department of Physics and Astronomy, Michigan State University, East Lansing MI, United States of America\\
$^{91}$ $^{(a)}$ INFN Sezione di Milano; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Milano, Milano, Italy\\
$^{92}$ B.I. Stepanov Institute of Physics, National Academy of Sciences of Belarus, Minsk, Republic of Belarus\\
$^{93}$ National Scientific and Educational Centre for Particle and High Energy Physics, Minsk, Republic of Belarus\\
$^{94}$ Department of Physics, Massachusetts Institute of Technology, Cambridge MA, United States of America\\
$^{95}$ Group of Particle Physics, University of Montreal, Montreal QC, Canada\\
$^{96}$ P.N. Lebedev Institute of Physics, Academy of Sciences, Moscow, Russia\\
$^{97}$ Institute for Theoretical and Experimental Physics (ITEP), Moscow, Russia\\
$^{98}$ National Research Nuclear University MEPhI, Moscow, Russia\\
$^{99}$ D.V. Skobeltsyn Institute of Nuclear Physics, M.V. Lomonosov Moscow State University, Moscow, Russia\\
$^{100}$ Fakult{\"a}t f{\"u}r Physik, Ludwig-Maximilians-Universit{\"a}t M{\"u}nchen, M{\"u}nchen, Germany\\
$^{101}$ Max-Planck-Institut f{\"u}r Physik (Werner-Heisenberg-Institut), M{\"u}nchen, Germany\\
$^{102}$ Nagasaki Institute of Applied Science, Nagasaki, Japan\\
$^{103}$ Graduate School of Science and Kobayashi-Maskawa Institute, Nagoya University, Nagoya, Japan\\
$^{104}$ $^{(a)}$ INFN Sezione di Napoli; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Napoli, Napoli, Italy\\
$^{105}$ Department of Physics and Astronomy, University of New Mexico, Albuquerque NM, United States of America\\
$^{106}$ Institute for Mathematics, Astrophysics and Particle Physics, Radboud University Nijmegen/Nikhef, Nijmegen, Netherlands\\
$^{107}$ Nikhef National Institute for Subatomic Physics and University of Amsterdam, Amsterdam, Netherlands\\
$^{108}$ Department of Physics, Northern Illinois University, DeKalb IL, United States of America\\
$^{109}$ Budker Institute of Nuclear Physics, SB RAS, Novosibirsk, Russia\\
$^{110}$ Department of Physics, New York University, New York NY, United States of America\\
$^{111}$ Ohio State University, Columbus OH, United States of America\\
$^{112}$ Faculty of Science, Okayama University, Okayama, Japan\\
$^{113}$ Homer L. Dodge Department of Physics and Astronomy, University of Oklahoma, Norman OK, United States of America\\
$^{114}$ Department of Physics, Oklahoma State University, Stillwater OK, United States of America\\
$^{115}$ Palack{\'y} University, RCPTM, Olomouc, Czech Republic\\
$^{116}$ Center for High Energy Physics, University of Oregon, Eugene OR, United States of America\\
$^{117}$ LAL, Universit{\'e} Paris-Sud and CNRS/IN2P3, Orsay, France\\
$^{118}$ Graduate School of Science, Osaka University, Osaka, Japan\\
$^{119}$ Department of Physics, University of Oslo, Oslo, Norway\\
$^{120}$ Department of Physics, Oxford University, Oxford, United Kingdom\\
$^{121}$ $^{(a)}$ INFN Sezione di Pavia; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Pavia, Pavia, Italy\\
$^{122}$ Department of Physics, University of Pennsylvania, Philadelphia PA, United States of America\\
$^{123}$ Petersburg Nuclear Physics Institute, Gatchina, Russia\\
$^{124}$ $^{(a)}$ INFN Sezione di Pisa; $^{(b)}$ Dipartimento di Fisica E. Fermi, Universit{\`a} di Pisa, Pisa, Italy\\
$^{125}$ Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh PA, United States of America\\
$^{126}$ $^{(a)}$ Laboratorio de Instrumentacao e Fisica Experimental de Particulas - LIP, Lisboa; $^{(b)}$ Faculdade de Ci{\^e}ncias, Universidade de Lisboa, Lisboa; $^{(c)}$ Department of Physics, University of Coimbra, Coimbra; $^{(d)}$ Centro de F{\'\i}sica Nuclear da Universidade de Lisboa, Lisboa; $^{(e)}$ Departamento de Fisica, Universidade do Minho, Braga; $^{(f)}$ Departamento de Fisica Teorica y del Cosmos and CAFPE, Universidad de Granada, Granada (Spain); $^{(g)}$ Dep Fisica and CEFITEC of Faculdade de Ciencias e Tecnologia, Universidade Nova de Lisboa, Caparica, Portugal\\
$^{127}$ Institute of Physics, Academy of Sciences of the Czech Republic, Praha, Czech Republic\\
$^{128}$ Czech Technical University in Prague, Praha, Czech Republic\\
$^{129}$ Faculty of Mathematics and Physics, Charles University in Prague, Praha, Czech Republic\\
$^{130}$ State Research Center Institute for High Energy Physics, Protvino, Russia\\
$^{131}$ Particle Physics Department, Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{132}$ Ritsumeikan University, Kusatsu, Shiga, Japan\\
$^{133}$ $^{(a)}$ INFN Sezione di Roma; $^{(b)}$ Dipartimento di Fisica, Sapienza Universit{\`a} di Roma, Roma, Italy\\
$^{134}$ $^{(a)}$ INFN Sezione di Roma Tor Vergata; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{135}$ $^{(a)}$ INFN Sezione di Roma Tre; $^{(b)}$ Dipartimento di Matematica e Fisica, Universit{\`a} Roma Tre, Roma, Italy\\
$^{136}$ $^{(a)}$ Facult{\'e} des Sciences Ain Chock, R{\'e}seau Universitaire de Physique des Hautes Energies - Universit{\'e} Hassan II, Casablanca; $^{(b)}$ Centre National de l'Energie des Sciences Techniques Nucleaires, Rabat; $^{(c)}$ Facult{\'e} des Sciences Semlalia, Universit{\'e} Cadi Ayyad, LPHEA-Marrakech; $^{(d)}$ Facult{\'e} des Sciences, Universit{\'e} Mohamed Premier and LPTPM, Oujda; $^{(e)}$ Facult{\'e} des sciences, Universit{\'e} Mohammed V-Agdal, Rabat, Morocco\\
$^{137}$ DSM/IRFU (Institut de Recherches sur les Lois Fondamentales de l'Univers), CEA Saclay (Commissariat {\`a} l'Energie Atomique et aux Energies Alternatives), Gif-sur-Yvette, France\\
$^{138}$ Santa Cruz Institute for Particle Physics, University of California Santa Cruz, Santa Cruz CA, United States of America\\
$^{139}$ Department of Physics, University of Washington, Seattle WA, United States of America\\
$^{140}$ Department of Physics and Astronomy, University of Sheffield, Sheffield, United Kingdom\\
$^{141}$ Department of Physics, Shinshu University, Nagano, Japan\\
$^{142}$ Fachbereich Physik, Universit{\"a}t Siegen, Siegen, Germany\\
$^{143}$ Department of Physics, Simon Fraser University, Burnaby BC, Canada\\
$^{144}$ SLAC National Accelerator Laboratory, Stanford CA, United States of America\\
$^{145}$ $^{(a)}$ Faculty of Mathematics, Physics {\&} Informatics, Comenius University, Bratislava; $^{(b)}$ Department of Subnuclear Physics, Institute of Experimental Physics of the Slovak Academy of Sciences, Kosice, Slovak Republic\\
$^{146}$ $^{(a)}$ Department of Physics, University of Cape Town, Cape Town; $^{(b)}$ Department of Physics, University of Johannesburg, Johannesburg; $^{(c)}$ School of Physics, University of the Witwatersrand, Johannesburg, South Africa\\
$^{147}$ $^{(a)}$ Department of Physics, Stockholm University; $^{(b)}$ The Oskar Klein Centre, Stockholm, Sweden\\
$^{148}$ Physics Department, Royal Institute of Technology, Stockholm, Sweden\\
$^{149}$ Departments of Physics {\&} Astronomy and Chemistry, Stony Brook University, Stony Brook NY, United States of America\\
$^{150}$ Department of Physics and Astronomy, University of Sussex, Brighton, United Kingdom\\
$^{151}$ School of Physics, University of Sydney, Sydney, Australia\\
$^{152}$ Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{153}$ Department of Physics, Technion: Israel Institute of Technology, Haifa, Israel\\
$^{154}$ Raymond and Beverly Sackler School of Physics and Astronomy, Tel Aviv University, Tel Aviv, Israel\\
$^{155}$ Department of Physics, Aristotle University of Thessaloniki, Thessaloniki, Greece\\
$^{156}$ International Center for Elementary Particle Physics and Department of Physics, The University of Tokyo, Tokyo, Japan\\
$^{157}$ Graduate School of Science and Technology, Tokyo Metropolitan University, Tokyo, Japan\\
$^{158}$ Department of Physics, Tokyo Institute of Technology, Tokyo, Japan\\
$^{159}$ Department of Physics, University of Toronto, Toronto ON, Canada\\
$^{160}$ $^{(a)}$ TRIUMF, Vancouver BC; $^{(b)}$ Department of Physics and Astronomy, York University, Toronto ON, Canada\\
$^{161}$ Faculty of Pure and Applied Sciences, University of Tsukuba, Tsukuba, Japan\\
$^{162}$ Department of Physics and Astronomy, Tufts University, Medford MA, United States of America\\
$^{163}$ Centro de Investigaciones, Universidad Antonio Narino, Bogota, Colombia\\
$^{164}$ Department of Physics and Astronomy, University of California Irvine, Irvine CA, United States of America\\
$^{165}$ $^{(a)}$ INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine; $^{(b)}$ ICTP, Trieste; $^{(c)}$ Dipartimento di Chimica, Fisica e Ambiente, Universit{\`a} di Udine, Udine, Italy\\
$^{166}$ Department of Physics, University of Illinois, Urbana IL, United States of America\\
$^{167}$ Department of Physics and Astronomy, University of Uppsala, Uppsala, Sweden\\
$^{168}$ Instituto de F{\'\i}sica Corpuscular (IFIC) and Departamento de F{\'\i}sica At{\'o}mica, Molecular y Nuclear and Departamento de Ingenier{\'\i}a Electr{\'o}nica and Instituto de Microelectr{\'o}nica de Barcelona (IMB-CNM), University of Valencia and CSIC, Valencia, Spain\\
$^{169}$ Department of Physics, University of British Columbia, Vancouver BC, Canada\\
$^{170}$ Department of Physics and Astronomy, University of Victoria, Victoria BC, Canada\\
$^{171}$ Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{172}$ Waseda University, Tokyo, Japan\\
$^{173}$ Department of Particle Physics, The Weizmann Institute of Science, Rehovot, Israel\\
$^{174}$ Department of Physics, University of Wisconsin, Madison WI, United States of America\\
$^{175}$ Fakult{\"a}t f{\"u}r Physik und Astronomie, Julius-Maximilians-Universit{\"a}t, W{\"u}rzburg, Germany\\
$^{176}$ Fachbereich C Physik, Bergische Universit{\"a}t Wuppertal, Wuppertal, Germany\\
$^{177}$ Department of Physics, Yale University, New Haven CT, United States of America\\
$^{178}$ Yerevan Physics Institute, Yerevan, Armenia\\
$^{179}$ Centre de Calcul de l'Institut National de Physique Nucl{\'e}aire et de Physique des Particules (IN2P3), Villeurbanne, France\\
$^{a}$ Also at Department of Physics, King's College London, London, United Kingdom\\
$^{b}$ Also at Institute of Physics, Azerbaijan Academy of Sciences, Baku, Azerbaijan\\
$^{c}$ Also at Novosibirsk State University, Novosibirsk, Russia\\
$^{d}$ Also at TRIUMF, Vancouver BC, Canada\\
$^{e}$ Also at Department of Physics, California State University, Fresno CA, United States of America\\
$^{f}$ Also at Department of Physics, University of Fribourg, Fribourg, Switzerland\\
$^{g}$ Also at Tomsk State University, Tomsk, Russia\\
$^{h}$ Also at CPPM, Aix-Marseille Universit{\'e} and CNRS/IN2P3, Marseille, France\\
$^{i}$ Also at Universit{\`a} di Napoli Parthenope, Napoli, Italy\\
$^{j}$ Also at Institute of Particle Physics (IPP), Canada\\
$^{k}$ Also at Particle Physics Department, Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{l}$ Also at Department of Physics, St. Petersburg State Polytechnical University, St. Petersburg, Russia\\
$^{m}$ Also at Louisiana Tech University, Ruston LA, United States of America\\
$^{n}$ Also at Institucio Catalana de Recerca i Estudis Avancats, ICREA, Barcelona, Spain\\
$^{o}$ Also at Department of Physics, National Tsing Hua University, Taiwan\\
$^{p}$ Also at Department of Physics, The University of Texas at Austin, Austin TX, United States of America\\
$^{q}$ Also at Institute of Theoretical Physics, Ilia State University, Tbilisi, Georgia\\
$^{r}$ Also at CERN, Geneva, Switzerland\\
$^{s}$ Also at Georgian Technical University (GTU),Tbilisi, Georgia\\
$^{t}$ Also at Ochadai Academic Production, Ochanomizu University, Tokyo, Japan\\
$^{u}$ Also at Manhattan College, New York NY, United States of America\\
$^{v}$ Also at Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{w}$ Also at LAL, Universit{\'e} Paris-Sud and CNRS/IN2P3, Orsay, France\\
$^{x}$ Also at Academia Sinica Grid Computing, Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{y}$ Also at Laboratoire de Physique Nucl{\'e}aire et de Hautes Energies, UPMC and Universit{\'e} Paris-Diderot and CNRS/IN2P3, Paris, France\\
$^{z}$ Also at Moscow Institute of Physics and Technology State University, Dolgoprudny, Russia\\
$^{aa}$ Also at Section de Physique, Universit{\'e} de Gen{\`e}ve, Geneva, Switzerland\\
$^{ab}$ Also at International School for Advanced Studies (SISSA), Trieste, Italy\\
$^{ac}$ Also at Department of Physics and Astronomy, University of South Carolina, Columbia SC, United States of America\\
$^{ad}$ Also at School of Physics and Engineering, Sun Yat-sen University, Guangzhou, China\\
$^{ae}$ Also at Faculty of Physics, M.V.Lomonosov Moscow State University, Moscow, Russia\\
$^{af}$ Also at National Research Nuclear University MEPhI, Moscow, Russia\\
$^{ag}$ Also at Department of Physics, Stanford University, Stanford CA, United States of America\\
$^{ah}$ Also at Institute for Particle and Nuclear Physics, Wigner Research Centre for Physics, Budapest, Hungary\\
$^{ai}$ Also at Department of Physics, The University of Michigan, Ann Arbor MI, United States of America\\
$^{aj}$ Also at Discipline of Physics, University of KwaZulu-Natal, Durban, South Africa\\
$^{ak}$ Also at University of Malaya, Department of Physics, Kuala Lumpur, Malaysia\\
$^{*}$ Deceased
\end{flushleft}

%% \end{document}
% Created with xml2latex.py

